Policy Choice in Time Series by Empirical Welfare Maximization

This paper develops a novel method for policy choice in a dynamic setting where the available data is a multivariate time series. Overcoming challenges unique to time-series setting such as time-varying environments, history-dependent welfare, dynamic causal effects, and statistical dependence, we propose Time-series Empirical Welfare Maximization (T-EWM) methods. We characterize conditions for T-EWM to consistently learn optimal policies conditional or unconditional on the time-series history, and derive nonasymptotic upper bounds for the welfare regrets. We illustrate a use of T-EWM for optimal restriction rules against Covid-19.

==> 3.3_Conti_Multi.tex <==

{\blue 
\subsubsection{Using unconditional T-EWM for multi-period decision}}

Using unconditional welfare can not only provide a faster convergence
rate of the conditional welfare regret, but it also leaves a decision
rule, which can be applied to future decision scenarios. Especially,
if the policy decision process, as is usually the case, exhibits a
certain degree of rigidity, then the policy rule, once established,
tends to govern decisions over a relatively extended future horizon.
The unconditional T-EWM will be particularly useful in these scenarios.

To illustrate this point, in this section, we consider a two-period
welfare target under a rigid decision rule, $G$:
\begin{align}
\mathcal{W}_{T:T+1}(G|\mathcal{F}_{T-1}) & =\mathsf{E}\left[\mathcal{W}_{T}(G|X_{T-1})+\mathcal{W}_{T+1}(G|X_{T})|X_{T-1}\right].\label{eq:two_p_wel_conti}
\end{align}
This welfare function can be straightforwardly extended to the finite multi-period case.
It should also be noted that the rigidity applies to the policy rule,
not to the individual policies themselves. Specifically, the planner
estimates the optimal policy rule, $\hat{G}$, using the data available
at the end of period $T-1$, and then implements it as
\begin{align}
W_{T} & =1(X_{T-1}\in\hat{G}),\nonumber \\
W_{T+1} & =1(X_{T}\in\hat{G}).\label{eq:two-p-policy}
\end{align}
i.e., at the end of period $T$, the planner observes the realized
$X_{T}$ and then makes the treatment choice in accordance with the
rule $\hat{G}$. Under this setup, an unconditional policy rule is
particularly meaningful. {\red Once a policy rule is obtained, it can be applied repeatedly to future treatment decisions while also incorporating updated information as it becomes available.} In the following, we show that, in such a scenario,
the estimated policy $\hat{G}$ given by \eqref{maxG} continues to be an
appropriate choice, since the regret of the aggregated welfare converges
at the same parametric rate as established in Theorem \ref{thm:mds_mean_bound}.

The welfare (\ref{eq:two_p_wel_conti}) can be written as
\begin{align}
\mathcal{W}_{T:T+1}(G|\mathcal{F}_{T-1}) & =\mathsf{E}\left[\mathcal{W}_{T}(G|X_{T-1})+\mathcal{W}_{T+1}(G|X_{T})|X_{T-1}\right]\nonumber \\
 & =\mathcal{W}_{T}(G|X_{T-1})+\mathsf{E}\left(\mathcal{W}_{T+1}(G|X_{T})|X_{T-1}\right)\nonumber \\
 & =\mathcal{W}_{T}(G|X_{T-1})+\mathsf{E}\left(\mathcal{W}_{T+1}(G|X_{T})\right),\label{eq:two-p-wefare_decomp}
\end{align}
where the first equality follows from Assumption \ref{ass:continuous_Markov}; the last
equality follows from the additional assumption that $X_{T-1}$ is
independent of $X_{T}$. Although this assumption is stronger than
those imposed in the previous sections, it can be satisfied in an
RCT setup, as well as those Bandit setups where previous choices and outcomes will not alter the subsequent data generating process. Comparable assumptions have also been employed in \cite{kasy2019adaptive} 
and \cite{cesa2025adaptive}. \footnote{In this section, we maintain this assumption. Its relaxation in the
multi-period setup is presented in Section \ref{sec_multi}, within the framework
of Section \ref{model_example}. A more general discussion of the multi-period
problem is provided in Section \ref{sec:connection}.}

For expositional clarity, we begin with the simplifying assumption
that the data are stationary, implying that for any $x\in\mathcal{X}$
and $G\in\mathcal{G}$, we have
\begin{equation}
\mathcal{W}_{T}(G|X_{T-1}=x)=\mathcal{W}_{T+1}(G|X_{T}=x).\label{eq:two_p_station}
\end{equation}
We relax the stationarity assumption later. By (\ref{eq:two_p_station})
and Assumption \ref{ass:correct_specify}., $G_{*}$ defined in \eqref{maxG} satisfies both
\begin{align}
G_{*} & \in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T}(G|X_{T-1}),\nonumber \\
G_{*} & \in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T+1}(G|X_{T-1}).\label{eq:two_p_opti}
\end{align}
Combining (\ref{eq:two-p-wefare_decomp}) and (\ref{eq:two_p_opti})
yields
\begin{align*}
\text{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T:T+1}(G|\mathcal{F}_{T-1}) & \leq\text{argmax}_{G_{1}\in\mathcal{G}}\mathcal{W}_{T}(G_{1}|X_{T-1})+\mathsf{E}\left(\text{argmax}_{G_{2}\in\mathcal{G}}\mathcal{W}_{T+1}(G_{2}|X_{T})\right)\\
 & =\mathcal{W}_{T}(G_{*}|X_{T-1})+\mathsf{E}\left(\mathcal{W}_{T+1}(G_{*}|X_{T})\right)=\mathcal{W}_{T:T+1}(G_{*}|\mathcal{F}_{T-1}),
\end{align*}
where the second equality follows from (\ref{eq:two_p_opti}). The
last row shows that $G_{*}$ is also the optimizer of $\mathcal{W}_{T:T+1}(\cdot|\mathcal{F}_{T-1})$.
This justifies applying $\hat{G}$, a well-behaved estimator of $G_{*}$
(see Theorem \ref{thm:mds_mean_bound_unconditional}), in the treatment choice procedure (\ref{eq:two-p-policy}).

Now, we relax the stationarity condition. Following (\ref{eq:two-p-wefare_decomp}),
\begin{align*}
\text{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T:T+1}(G|\mathcal{F}_{T-1}) & \leq\text{argmax}_{G_{1}\in\mathcal{G}}\mathcal{W}_{T}(G_{1}|X_{T-1})+\mathsf{E}\left(\text{argmax}_{G_{2}\in\mathcal{G}}\mathcal{W}_{T+1}(G_{2}|X_{T})\right)\\
 & =\mathcal{W}_{T}(G_{T}^{*}|X_{T-1})+\mathsf{E}\left(\mathcal{W}_{T+1}(G_{T+1}^{*}|X_{T})\right),
\end{align*}
where we define $G_{T}^{*}\in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T}(G)$
and $G_{T+1}^{*}\in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T+1}(G)$
in the last equality, and the last equality follows from Assumption \ref{ass:correct_specify}.

Rather than imposing stationarity, we extend Assumption \ref{equiv_W_uc} to:
for any $G\in\mathcal{G}$, there exists some constant $c$, such
that
\begin{align}
\mathcal{W}_{T}(G_{T}^{*})-\mathcal{W}_{T}(G) & \leq c\big[\widetilde{\mathcal{W}}(G_{T}^{*})-\widetilde{\mathcal{W}}(G)\big],\nonumber \\
\mathcal{W}_{T+1}(G_{T+1}^{*})-\mathcal{W}_{T+1}(G) & \leq c\big[\widetilde{\mathcal{W}}(G_{T+1}^{*})-\widetilde{\mathcal{W}}(G)\big],\label{eq:extended welfare ordering}
\end{align}
where $\widetilde{\mathcal{W}}(G)$ is the same intermediate welfare
defined in \eqref{2intermediate_welfare}, constructed using the data available up to time
$T-1$. This extension of Assumption \ref{equiv_W_uc}  is natural, since the planner
is required to specify a rigid decision rule for both $T$ and $T+1$,
at the end of time $T-1$. We would like to emphasize that in a decision
problem, where a planner makes a future decision based on the historical
data, an assumption linking the past and the future is always necessary.
In the time series literature, a widely adopted assumption of this
type is stationarity (or a structural model that accommodates certain
forms of non-stationarity). One of the main contributions of this
paper is to considerably relax the stationarity assumption in causal
inference for time series, by proposing the model-free assumptions of invariance of the welfare ordering, including Assumpitons 
\ref{equiv_W}, \ref{equiv_W_c}, \ref{equiv_W_uc}, and their variants. 

Although $G_{T}^{*}$ and $G_{T+1}^{*}$ may differ in the absence
of stationarity, (\ref{eq:extended welfare ordering}) ensures that,
under the treatment choice (\ref{eq:two-p-policy}), the aggregated
welfare regret from both periods converges at a similar parametric
rate as established in Theorem \ref{thm:mds_mean_bound}.




==> 3.3s_Conti_Multi.tex <==

{\blue 
\subsubsection{Using unconditional T-EWM for multi-period decision}}

Using unconditional welfare can not only provide a faster convergence
rate of the conditional welfare regret, but it also leaves a decision
rule, which can be applied to future decision scenarios. Especially,
if the policy decision process, as is usually the case, exhibits a
certain degree of rigidity, then the policy rule, once established,
tends to govern decisions over a relatively extended future horizon.
The unconditional T-EWM will be particularly useful in these scenarios.

Consider a two-period
welfare target under a rigid decision rule, $G$:
\begin{align}
\mathcal{W}_{T:T+1}(G|\mathcal{F}_{T-1}) & =\mathsf{E}\left[\mathcal{W}_{T}(G|X_{T-1})+\mathcal{W}_{T+1}(G|X_{T})|X_{T-1}\right].\label{eq:two_p_wel_conti}
\end{align}
This welfare function can be straightforwardly extended to the finite multi-period case.
It should also be noted that the rigidity applies to the policy rule,
not to the individual policies themselves. Specifically, the planner
estimates the optimal policy rule, $\hat{G}$, using the data available
at the end of period $T-1$, and then implements it as
\begin{equation}
W_{T}  =1(X_{T-1}\in\hat{G}), \quad W_{T+1}  =1(X_{T}\in\hat{G}).
\label{eq:two-p-policy}
\end{equation}
i.e., at the end of period $T$, the planner observes the realized
$X_{T}$ and then makes the treatment choice in accordance with the
rule $\hat{G}$.{\color{blue} When decisions span multiple periods, restricting attention to a simple binary treatment, as in the one-period conditional welfare function, is no longer adequate. In such cases, richer decision rules and the analysis of the unconditional welfare function are required.}


{\color{red}Furthermore, we extend Assumption \ref{equiv_W_uc} (Invariance of the welfare ordering) to:
for any $G\in\mathcal{G}$, there exists some constant $c$, such
that
\begin{align}
	\mathcal{W}_{T}(G_{T}^{*})-\mathcal{W}_{T}(G) & \leq c\big[\widetilde{\mathcal{W}}(G_{T}^{*})-\widetilde{\mathcal{W}}(G)\big],\nonumber \\
	\mathcal{W}_{T+1}(G_{T+1}^{*})-\mathcal{W}_{T+1}(G) & \leq c\big[\widetilde{\mathcal{W}}(G_{T+1}^{*})-\widetilde{\mathcal{W}}(G)\big],\label{eq:extended welfare ordering}
\end{align}
where we define $G_{T}^{*}\in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T}(G)$
and $G_{T+1}^{*}\in\mbox{argmax}_{G\in\mathcal{G}}\mathcal{W}_{T+1}(G)$, and $\widetilde{\mathcal{W}}(G)$ is the same intermediate welfare
defined in \eqref{2intermediate_welfare}, constructed using the data available up to time
$T-1$. This extension of Assumption \ref{equiv_W_uc}  is natural, since the planner
is required to specify a rigid decision rule for both $T$ and $T+1$,
at the end of time $T-1$. 

It can be shown that 
the estimated policy $\hat{G}$ given by \eqref{maxG} continues to be an
appropriate choice, under the additional assumption that $X_{T-1}$ is
independent of $X_{T}$. Although this assumption is stronger than
those imposed in the previous sections, it can be satisfied in an
RCT setup, as well as those Bandit setups where previous choices and outcomes will not alter the subsequent data generating process. Comparable assumptions have also been employed in \cite{kasy2019adaptive} 
and \cite{cesa2025adaptive}.\footnote{ Its relaxation in the
	multi-period setup is presented in Section \ref{sec_multi}, within the framework
	of Section \ref{model_example}. A more general discussion of the multi-period
	problem is provided in Section \ref{sec:connection}.} As a result, an unconditional policy rule is particularly meaningful in this scenario.} {\red Once a policy rule is obtained, it can be applied repeatedly to future treatment decisions while also incorporating updated information as it becomes available.} 

==> 5.2.2_multiple_extension.tex <==

\subsubsection{Extended model: an example}
In this subsection, we discuss a possible further extension of the two-period case of the previous subsection.
Recall that we assume that we can update information at $T+1$ by conditioning on $g_1(W_{T-1})$. When this is not possible, a one-off
multiple-period decision is adopted. However, this typically requires us to relax the Markov properties specified in  Assumption \ref{ass:toy_example}, as
we need to ensure a path of treatment variables to be conditionally independent given the historical path. In addition, we also extend the exclusion condition by adding one more order of $W_t$.
%
% Relaxing the following conditions imposed on the simple model will considerably complicate the structure
% \begin{itemize}
	% \item[(i)] Relaxing the exclusion condition \eqref{exclu2}.
	% \item[(ii)] Allowing continuous covariates be in the model.
	% \item[(iii)] Allowing future decisions being based on the future covariate.
	%  \end{itemize}
%Here we only discussed the extension (i).

Namely, we relax Assumption  \ref{ass:toy_example} to,
\begin{align}
	Y_{t}(w_{0:t}) & =Y_{t}(w_{t-2,}w_{t-1},w_{t})\nonumber, \\
	Y_{t}(w_{0:t}) & \perp W_{0:t-2}|W_{t-2},W_{t-1}\nonumber, \\
	W_{t} & \perp X_{0:t-2}|W_{t-2},W_{t-1}\label{eq:relaxed_exclu},
\end{align}
where we assume that the conditional independence of $W_{t-1}: W_{t-2}$.
In the remainder of this section we use the following abbreviations $g_1:=g_1(W_{t-1})$.
We shall decompose
\begin{align*}
	&\mathcal{W}_{T:T+1}(g_{1}(.) ,g_{2}(.) |w),\\
	&=  \E\left[Y_{T}(W_{T-2},W_{T-1},g_{1}(W_{T-1}) )+Y_{T+1}(W_{T-1},g_{1}(W_{T-1}) ,g_{2}(W_{T}) )|W_{T-1}=w\right],\\
	&=  \E\left[Y_{T}(W_{T-2},W_{T-1},g_{1}(W_{T-1}) )|W_{T-1}=w\right]+\E\left[Y_{T+1}(W_{T-1},g_{1}(W_{T-1}) ,g_{2}(W_{T}) )|W_{T-1}=w\right],\\
	&=  I+II.
\end{align*}
Under Assumption \ref{ass:toy_example} we should have
\begin{align*}
	I & =\E\left[Y_{T}(W_{T-1},g_{1}(W_{T-1}) )|W_{T-1}=w\right],\\
	& =\E\left\{ Y_{T}(W_{T-1},1)g_{1}(W_{T-1}) +Y_{T}(W_{T-1},1)\left(1-g_{1}(W_{T-1}) \right)|W_{T-1}=w\right\},\\
	II & =\E\left[Y_{T+1}(W_{T-1},W_{T},g_{2}(W_{T}) )|W_{T}=g_{1}(W_{T-1}) ,W_{T-1}=w\right],\\
	& =\E\left[Y_{T+1}(W_{T},g_{2}(W_{T}) )|W_{T}=g_{1}(w) \right],\\
	& =\E\left\{ Y_{T+1}(W_{T},1)g_{2}(W_{T}) +Y_{T+1}(W_{T},1)\left(1-g_{2}(W_{T}) \right)|W_{T}=g_{1}(w) \right\} .
\end{align*}
Then it is the same equation as in \eqref{eq:multi_welfare}. Now, with the relaxed Markov properties in (\ref{eq:relaxed_exclu}), we have
\begin{align*}
	I & =\E\left[Y_{T}(W_{T-2},W_{T-1},g_{1}(W_{T-1}) )|W_{T-1}=w\right],\\
	& =\E\left\{ Y_{T}(W_{T-2},W_{T-1},1)g_{1}(W_{T-1}) +Y_{T}(W_{T-2},W_{T-1},1)\left(1-g_{1}(W_{T-1}) \right)|W_{T-1}=w\right\} .
\end{align*}

Its empirical analogue is
\begin{align}
	& \frac{1}{T(w)}\sum_{W_{t-1}=w}\left\{ \frac{Y_{t}W_{t}g_{1}(W_{t-1}) }{\text{Pr}(W_{t}=1|W_{t-1}=w)}+\frac{Y_{t}\left(1-W_{t}\right)\left(1-g_{1}(W_{t-1}) \right)}{1-\text{Pr}(W_{t}=1|W_{t-1}=w)}\right\} .\label{eq:relaxed_T_sample}
\end{align}
It is the same as the first term of \eqref{sample_multi}. However, $II$ becomes
\begin{align*}
	II & =\E\left[Y_{T+1}(W_{t-1},g_{1}(W_{T-1}),g_{2}(W_{T}))|W_{T-1}=w\right]\\
	& =\E\left\{ \sum_{(w_{T},w_{T+1})\in\{0,1\}^{2}}Y_{T+1}(W_{T-1},w_{T},w_{T+1})1(w_{T}=g_{1}(W_{T-1}) ,w_{T+1}=g_{2}(W_{T}))|W_{T-1}=w\right\}.
\end{align*}
A valid sample counterpart of II can be
\begin{align} \label{eq: sample_path}
	& \frac{1}{T(w)}\sum_{W_{t-2}=w}\left\{ \frac{Y_{t}1(W_{t-1}=g_{1}(W_{t-2}) ,W_{t}=g_{2}(W_{t-1}) )}{\text{Pr}(W_{t}=g_{2}(W_{t-1}) ,W_{t-1}=g_{1}(W_{t-2}) |W_{t-2}=w)}\right\} \nonumber, \\
	= & \frac{1}{T(w)}\sum_{W_{t-2}=w}\left\{ \frac{Y_{t}1(W_{t-1}=g_{1}(W_{t-2}) )1(W_{t}=g_{2}(W_{t-1}) )}{\text{Pr}(W_{t}=g_{2}(W_{t-1}) |W_{t-1}=g_{1}(W_{t-2}) ,W_{t-2}=w)\text{Pr}(W_{t-1}=g_{1}(W_{t-2}) |W_{t-2}=w)}\right\}.
\end{align}
This is more complicated than the second term of \eqref{sample_multi}. A major difference between them is number of observations. The second term of \eqref{sample_multi}
has $\#\{W_{t-1}=g_{1}(w) ,W_{t}=g_{2}(W_{t-1}) \}$ but \eqref{eq: sample_path} has $\#\{W_{t-2}=w,W_{t-1}=g_{1}(W_{t-2}) ,W_{t}=g_{2}(W_{t-1}) \}$ due to the extension of the exclusion condition.
The sample size decreases with the increase of the order of the time series.
Moreover, the denominator of (\ref{eq: sample_path}) tends to be smaller, which likely results in a
large variance.


==> 5.3_multi_lag.tex <==

\subsection{Multiple lags} \label{multi-lag}
In this subsection, we discuss the extension to a $p$ lag policy decision framework.
Suppose that the planner choose treatment at time $T$ to  maximize the expected welfare at time $T+p$. Thus the policy choice depends on the quantification of a $p-$ lag causal effects. For simplicity, we base our discussion on the simple discrete model discussed in Section \ref{one-p}.
{\color{red} (NEED DISCUSSION here, should we simply let q=1)
Namely, for an integer $q$, we relax the Assumption  \ref{ass:toy_example} to,
\begin{align}
	Y_{t+p}(w_{0:t}) & =Y_{t+p}(w_{t-1:t})\nonumber, \\
	Y_{t+p}(w_{0:t}) & \perp W_{0:t-1}|W_{t-1}\nonumber, \\
	W_{t} & \perp X_{0:t}|W_{t-1}\label{eq:relaxed_exclu}.
\end{align}
}
A $p-$ lag conditional welfare function can be denoted as,
\bea \label{p-lag1}
\mathcal{W}_{T,p}(g|W_{T-1})
&=&\E\bigg\{ Y_{T+p}(W_{T-1},1,W_{T+1:T+p}) g(W_{T-1})\nonumber \\
&&+Y_{T+p}(W_{T-1},0,W_{T+1:T+p})\left( 1-g(W_{T-1})\right) )
|W_{T-1:T-q}\bigg\}.
\eea
Another choice of a welfare function can be of a weighted $p-$ lag form,
\begin{eqnarray}  \label{p-lag2}
        \mathcal{W}_{T,p}(g|W_{T-1})
        =  \E \left\{ \begin{array}{c}
                \sum_{w\in(0,1)^{p}}a_{w}\big[Y_{T+p}(W_{T-1},1,w)g(W_{T-1})\\
                +Y_{T+p}(W_{T-1},0,w)[ 1-g(W_{T-1})] \big]
        \end{array}\bigg|W_{T-1:T-q}\right\},
\end{eqnarray}

where $w\in\{0,1\}^p$ and $a_w$ is a weight function specified by the planner.

{
        (\ref{p-lag2}) is a natural extension of the p-lag treatment effect in \cite{bojinov2019time}. Note that (\ref{p-lag1}) can be regarded as a special case of (\ref{p-lag2}) with
        $$P(W_{T+1:T+p}=w|W_{T-1},W_T=1)=P(W_{T+1:T+p}=w|W_{T-1},W_T=0)\defeq a_w.$$
        Therefore, we focus on (\ref{p-lag2})}.
Accordingly, we extend
{\bf Assumption \ref{bound1}} to \\
\textit{For every $t\in \mathbb{N}$ any $w\in \{0,1\}^{p+1}$, there exists $\kappa \in (0,1/2)$, such that
        \begin{equation*}
                \kappa \leq \Pr(W_{t:t+p}=w|W_{t-1}) \leq 1-\kappa.
        \end{equation*}
        for each $x\in\mathcal{X}$.}

Assumption \ref{unconf} must also be extended to fit with the multiple lag framework.
{\color{red}
\begin{assumption} \label{unconf_p}
        for any $t\in \mathbb{N}$ and $w\in \{0,1\}^{p+1}$
        \begin{equation}
                Y_{t+p}(W_{t-1},w)\perp W_{t}|W_{t-1:t-q-1}.
        \end{equation}
\end{assumption}}

Following the notation of \cite{bojinov2019time}, let $W_{t_1:t_2}$ be the random path of treatments, starting from time $t_1$ and ending at time $t_2$. Let $w\in \{0,1\}^{p+1}$ and $w^{\prime}\in\{0,1\}^{p+1}$, then the sample counterpart of (\ref{p-lag2}) can be,
\bea \label{sample_conti}
\hat{\mathcal{W}}_{p}(g|w^{\prime})
&=&\frac{1}{T(w^{\prime})}\sum_{t : t<T-p, \; W_{t-1} = w^{\prime}}
\sum_{w\in\{0,1\}^{p}}a_w\bigg\{\frac{Y_{t+p}\mathbf{1}\{W_{t:t+p}=(1,w)\}}{e_{t}(1,w)} g(W_{t-1})\nonumber\\
&+& \frac{Y_{t+p}\mathbf{1}\{W_{t:t+p}=(0,w)\}}{e_{t}(0,w)}[ 1-g(W_{t-1}) ] \bigg\},
\eea
where $e_{t}(1,w):=\Pr(W_{t:t+p}=1:w|W_{t-1}, Y_{t:t+p}(\cdot))$, with $Y_{t:t+p}(\cdot)$ as the counterfactual outcomes of all the paths from $t$ to $t+p$. We refer to Section 4 of \cite{bojinov2019time} to the details of propensity score conditional on this type of filtration.
%Similarly to Chapter \ref{discrete_bound}, let define
%{\small \begin{eqnarray} \label{multi_E1}
%               &&\bar{\mathcal{W}}_{p}(g|w^{\prime})\\
%               & = & \frac{1}{T(w^{\prime})}\sum_{t : t<T-p, \; W_{t-1} = w^{\prime}}
%               \E\left\{ \begin{array}{c}
%                       \sum_{w\in(0,1)^{p}}a_{w}
%                       \big[Y_{t+p}(w_{1:t-1}^{obs},1,w) g(W_{t-1})\\
%                       +Y_{t+p}(w_{1:t-1}^{obs},0,w)[ 1-g(W_{t-1}) ]\big]
%               \end{array}\bigg|W_{t-1}=w^{\prime}\right\}\nonumber.
%\end{eqnarray}}
%{[Problem with the Assumption \ref{unconf} in the p-lag case]} With Assumption \ref{bound1} and \ref{unconf} modified for the p-lag case, we have $\hat{\mathcal{W}}_{p}(G^{(1)}|G^{(2)})-\bar{\mathcal{W}}_{p}(G^{(1)}|G^{(2)})$ being a martingale difference series. However, with $p>0$, the  unconfoundedness condition (\ref{unconf_p}) implies that $X_{t:t+p-1}$ cannot be related on $W_{t:t+p}$. This might exclude many dependence structures. \footnote{From MX: After a follow-up discussion with Weining, we still think in certain cases the framework of BS is unavoidable, we will refine this points after more discussions.}
%
%An alternative $\bar{\mathcal{W}_p}$ is
%{\small \begin{eqnarray} \label{multi_E2}
%               &&\bar{\mathcal{W}}^2_{p}(G^{(1)}|G^{(2)})\\
%               & = & T(G^{(2)})^{-1}\sum_{t : t<T-p, \; X_{t-1}^{(2)} \in G^{(2)}}
%               {\E}^R\left\{ \begin{array}{c}
%                       \sum_{w\in(0,1)^{p}}a_{w}
%                       \big[Y_{t+p}(w_{1:t-1}^{obs},1,w)\mathbf{1}\{X^{(1)}_{t-1}\in G^{(1)}\}\\
%                       +Y_{t+p}(w_{1:t-1}^{obs},0,w)\mathbf{1}\{X^{(1)}_{t-1} \not\in G^{(1)}\}\big]
%               \end{array}\bigg|X_{t-1}\right\}\nonumber,
%\end{eqnarray}}
%where $\E{^{R}}(\cdot)=\E(\cdot|Y_{1:T}(.))$, and $Y_{1:T}(.)$ is the collection of all the potential paths of outcomes up to time $T$. This structure is proposed by \cite{bojinov2019time} for the estimation of dynamic average treatment effect. With (\ref{multi_E2}), we no longer need Assumption \ref{unconf}, but we need the following one
%{  \small \begin{assumption}\label{treat3} (Non-anticipating treatment)
%               \begin{equation}
%                       \P(W_{t}=w_{t}|W_{1:t-1}=w,Y_{1:T}(.))=\P(W_{t}=w_{t}|W_{1:t-1}=w,Y_{1:t-1}(w)).
%               \end{equation}
%               For any $w$ and $z$.
%       \end{assumption}
%}
%and
%\beaa
%g^*(w^{\prime}) &=& \mbox{argmax}_{g: \{w^{\prime}\}\to  \{0,1\}} \mathcal{W}_{T,p}(g|w^{\prime}),\\
%\hat{g}(w^{\prime}) &=& \mbox{argmax}_{g: \{w^{\prime}\}\to  \{0,1\}} \hat{\mathcal{W}}_{p}(g|w^{\prime}).
%\eeaa
%{\bf Assupmtion \ref{equiv_W}} is modified to
%
%\textit{For any $g_1$, $g_2\in \{0,1\}\to \{0,1\}$, and $w^{\prime}\in  \{0,1\}$.
%       \beqq
%       \mathcal{W}_{T,p}(g|w^{\prime})- \mathcal{W}_{T,p}(g|w^{\prime}) \leq c\big[\bar{\mathcal{W}}_p(g|w^{\prime})-\bar{\mathcal{W}}_p(g|w^{\prime})\big],
%       \eeqq
%       with probability approaching one.}
%Let $\bar{\mathcal{W}}_{p}$ be either $\bar{\mathcal{W}}^1_{p}$ or $\bar{\mathcal{W}}^2_{p}$.
%Under Assumption \ref{unconf_p}, $\hat{\mathcal{W}}_{p}(g|w^{\prime})-\bar{\mathcal{W}}_{p}(g|w^{\prime})$ is a sum of MDS.
 It shall be noted that, by similar arguments to Section \ref{discrete_bound} and \ref{sec:uncon_con}, we can show that the upper bound of $\mathcal{W}_{T,p}(g^*|w^{\prime})-\mathcal{W}_{T,p}(\hat{g}|w^{\prime})$ is converges uniformly at the rate $\frac{1}{\sqrt{T-p-1}}$.

==> 6.1_lower_bound.tex <==
\subsection{Minimax lower bound} \label{L_b}

We now prove the lower bound of the risk of the proposed method. We follow the proof strategy
of Theorem 3 in \citet{devroye1995lower}, which is based on Hellinger distances.

\begin{theorem} \label{th:lower_bound}
	Assume Assumptions \ref{unconf}, \ref{bound1}, \ref{bound_c} and \ref{cover1}, we have the following lower bound,
	\beq
	\underset{P_T\in\mathcal{P}(M,\kappa)}{\text{sup}}{\E}_{P_T}\{\mathcal{W}(G_{*})-\mathcal{W}(\hat{G})\}\geq\sqrt{v/(T-1)}\exp(-1).
	\eeq
%	where $\underline{p}_{2}$ is a constant depending on the dependency of the specified process.
\end{theorem}
A proof is presented in Appendix \ref{sec: proof_lower}. This theorem and Theorem \ref{thm:mds_mean_bound} together show the minimax optimality of the proposed T-EWM method.

%We shall now bound the conditional welfare below by the unconditional welfare function. Assume we have bounded support of $X_{T-1}$, $B$. Note we have for constant $C_B$
%Assume that $x$ is of a bounded support, moreover, we assume that there exist constants $C_B$ $c$ we have $f(x_{\max})\leq c f(x_{obs})$, and $f(x)$ is bounded from below on a bounded support.
%Then we can bound the unconditional welfare from the above by the conditional welfare function.
%\begin{eqnarray}
%	&&\int_B R_T(x, G) f_{X_{T-1} }(x) dx \nonumber \\
%	&&\leq C_B R_T(x_{\max}, G)  f_{X_{T-1}}(x_{\max}),
	%&&\leq  C_B  c  R_T(x_{obs}, G)f_{X_{T-1}^{(2)}}(x_{obs}),
%\end{eqnarray}
%where $x_{\max}$ is the value at which attached maximum for the function $ R_T(x, G) f_{X_{T-1}^{(2)}}(x) $.
%Then we have the above results translated to the (worst-case) conditional welfare function.
%Define the set $B(x_{obs})= \IF\{x:R_T(x, G)>R_T(x_{obs},G)\}$, so we have
%
%\begin{eqnarray}
%	&&\int_B R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx, \nonumber \\
%	&&\leq \int_{B(x_{obs})} R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx+\int_{B(x_{obs})^c} R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx,\\
%	&&\leq \int_{B(x_{obs})} R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx + C_B R_T(x_{obs}, G) f_{X_{T-1}^{(2)}}(x_{obs}).
%	%&&\leq  C_B  c  R_T(x_{obs}, G)f_{X_{T-1}^{(2)}}(x_{obs}),
%\end{eqnarray}
%
%So we have
%\begin{eqnarray}
%	&&\int_{B(x_{obs})^c} R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx, \nonumber \\
%	&&\leq  C_B R_T(x_{obs}, G) f_{X_{T-1}^{(2)}}(x_{obs}).
%\end{eqnarray}
%Thus we have
%
%
%\begin{eqnarray}
%	&&\int R_T(x, G) f_{X_{T-1}^{(2)} }(x) dx, \nonumber \\
%	&&\leq  2C_B R_T(x_{obs}, G) f_{X_{T-1}^{(2)}}(x_{obs}).
%	%&&\leq  C_B  c  R_T(x_{obs}, G)f_{X_{T-1}^{(2)}}(x_{obs}),
%\end{eqnarray}


==> 6.1_marginal.tex <==
\subsection{Improved rates with margin assumption} \label{improved_rate}

In this section, we show special cases where we can improve the rate by imposing additional margin assumptions. Here we maintain the setting and method of Section \ref{sec:uncon_con}. In particular, we assume that the first best policy is feasible, and we bound conditional regret with unconditional regret.

For simplicity, we assume that $X_{t}=\{Y_t,W_t\}$ are strictly stationary. We also use the compact notation $Y_t(W_{1:t-1},1)  = Y_t(1)$ and $Y_t(W_{1:t-1},0)  = Y_t(0)$. Define
\beqq
\tau(W_{t-1})=\E((Y_t(1)- Y_t(0))|W_{t-1}).
\eeqq
If we are willing to make stronger assumptions, such that observations have very small probabilities to fall into a small region near the margin of the above optimal classification region, we can potentially achieve a better rate. For a detailed insight in the i.i.d. case, see, for example, \cite{boucheron2005theory}.
Let
\beaa 
\bar{\mathcal{W}}(g,W_{t-2}) 
&=&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\E\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]|W_{t-2}\right\}. \notag \\
%\label{eq:W2appendix}
\bar{\mathcal{W}}(g) &=&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\E\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]\right\}. \notag \\
{\widehat{\mathcal{W}}}(g) 
&=&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]\right\}. \notag 
\eeaa

We shall assume that
\begin{assumption}	\label{C.1} The first best treatment rule $g^*_{\text{FB}}$  belongs to the class of candidate treatment rules
	$g$,  i.e., $g^*_{\text{FB}}=g^*$.
	\end{assumption}
	\begin{assumption}
	\label{C.2} The class of treatment rules is finite and countable with $|\mathcal{G}| = 2 \lesssim n^V$, where $V$ is a fixed integer.
	\end{assumption}
	\begin{assumption}\label{C.3} $Y_t(0), Y_t(1)$ belong to $[-C,C]$, where $C$ is a constant.\end{assumption}
	\begin{assumption}\label{C.4} The following margin condition is assumed. Let $\Pr_{t-1}$ be 
	$\Pr(.| \mathcal{F}_{t-2})$.
	There exists a constant $0 \leq \eta \leq C$, $0 < \alpha<\infty$ and $0\leq u\leq \eta$, such that
	\begin{eqnarray}
		\max_t \Pr{_{t-1}}(|\tau(W_{t-1})|\leq u ) \leq (u/\eta)^{\alpha}, \quad \quad \forall 0 \leq u\leq \eta.
	\end{eqnarray}
	The above assumption can be implied in the discrete case by the condition that there exists a positive constant $c$ such that $\tau(0),\tau(1)> c$. Pick $\eta = c$. Then, we have $\alpha = \infty$, $\P_{t-1}(|\tau(W_{t-1})|\leq u )  = 0,\quad \forall 0 \leq u\leq \eta$, and 
$\P_{{t-1}}(\cdot)=\text{Pr}(\cdot| {\mathcal{F}}_{t-2})$. 
	Recall that  there exists a positive constant $\overline{P} $  such that $ \frac{1}{T-1}\sum_t \P_{{t-1}} (g^*(W_{t-1})\neq g(W_{t-1}))\geq \overline{P} $.
	\end{assumption}
 \begin{assumption}\label{C.5}
$\Pr(.| W_{t-2})$ and $\Pr(.| W_{t-1})$ are strictly positive.
\end{assumption}
	
	

\begin{theorem} \label{lem: marginal_improve}
	Under Assumption \ref{C.1}-\ref{C.5} and Assumption \ref{unconf_c} , for a small enough positive $\delta>0$, we have the following bound with probability $1-\delta$,
	\beqq
	 \bar{\mathcal{W}}(g^*)- 	\bar{\mathcal{W}}(\hat{g})  \lesssim_p  C_{\alpha,\eta, V} (\frac{\sqrt{\log (2T/\delta)}}{\sqrt{T-1}})^{2(\alpha+1)/(\alpha+2)},
	\eeqq
	where $C_{\alpha,\eta, V}$ is a constant depending only on $\alpha$, $\eta$, and $V$.
\end{theorem}
We can see that when $\alpha = 0$, the rate becomes $\frac{1}{\sqrt{T-1}} \sqrt{\log 2T/\delta}$, which means that it has almost no constraint.  When $\alpha  \to \infty $, it is approaching $\frac{1}{T-1}\sqrt{\log 2T/\delta}$ (the best rate). Then, with the arguments in Section \ref{sec:uncon_con} we can bound the conditional regret. A proof is in Appendix \ref{sec: proof_marginal}.

==> 8_application.tex <==
\section{Application} \label{applica}

In this section, we illustrate the usefulness of T-EWM with an empirical application. 
Maintaining low unemployment rate,
stable inflation rate, and rapid economic growth are the ultimate goals of a central bank. How monetary policy,
such as changes in the FOMC target rate, can affect macroeconomic
targets, has been extensively studied. See, e.g.,
\cite{romer1989does}, \cite{bagliano1998measuring}, \cite{christiano1999monetary}, and many
others. On the other hand, the finance literature documents an increase in the
equity premium following Federal Open Market Committee (FOMC) meetings. In particular,\cite{lucca2015pre} find that
The next lemma concerns the tail probability bound. It states that, under certain regularity
conditions, | E nh|Hn is very close to E(| E nh|Hn ).
LEMMA A.4. Under Assumption 3.2, 3.3, and 3.7 to 3.9,
| E nh|Hn − E(| E nh|Hn ) ≲p M cn
√v/n,
where cn is arbitrarily slowly growing sequence.
Proof. Similar to the above derivation, for a positive constant ηk, with ∑
k ηk ≤ 1,
Pr(n−1
n∑
t=1
ht ≥ x)
≤ Pr(n−1|
K∑
k=1
n∑
t=1
h(k)
t − h(k−1)
t | ≥ x − √n−12−K M )
≤
K∑
k=1
Pr(|n−1
n∑
t=1
h(k)
t − h(k−1)
t | ≥ ηk(x − √n−12−K M ))
≤
K∑
k=1
exp{log max
t sup
Q
N 2(2−kM, Ht, ∥.∥Q,2) − η2
k(nx − √n2−K M )2/[2{(nx − √n2−K M )
+2((3 · 2−k · M )2n)}]}
≤
K∑
k=1
exp(log(K) + log(v + 1) + (v + 1)(log 4 + 1) + (2v) log( 2
2−kM )
−η2
k(nx − √n2−K M ))2/(2((nx − √n2−K M ) + 2((3 · 2−k · M )2n))),
where the above derivation is due to the tail probability in Lemma A.1. We pick ηk and x
to ensure the right hand side converges to zero and ∑
k ηk ≤ 1.
We take bk = log(K) + log(v + 1) + (v + 1)(log 4 + 1) + (2v) log( 2
2−k M ), ak = 2−1(nx −
√n2−K M ))2/((nx−√n2−K M )+2((3∗2−k ∗M )2n)). We pick ηk ≥ √ak/bk, so that bk ≤ η2
kak.
We also need to choose x to ensure that ∑
k ηk ≤ 1 and ∑
k exp(bk − η2
kak) → 0. We pick
cn
√v/n ≲ x, and ηk = c′
n
√bk/ak, with two slowly growing functions cn and c′
n and c′
n ≪ cn.
We set x = E(| E nh|Hn ) + cn
√v/n. The result then follows.
Finally, Theorem 3.1 follows from combining Lemma A.3, Lemma A.4, and n = T − 1.
56
A.4 Justifying Assumption 3.8
Here we now intepret the entropy condition in Assumption 3.8. We follow the argument of
Chapter 11 in Kosorok (2008) for the functional class related to non-i.i.d. data.
First, we illustrate the case that the random stochastic process {Dt}∞
t=−∞
def
= {Yt, Wt, Xt−1}∞
t=−∞
is assumed to be stationary. In this case, we have for all t ∈ {1, 2, . . . , n},
ht(·; G) = h(·; G)
and H = {h(·; G) = ̂ Wt(G) −  ̄Wt(G) : G ∈ G}.
For a n-dimensional non-negative vector αn = {αn,1, αn,2, . . . , αn,n}, define Qαn as a dis-
crete measure with probability mass αn,t
∑n
t=1 αn,t on the value Dt. Recall for a function f , its
Lr(Q)−norm is denoted by ||f ||Q,r
def
= [ ́
v |f (v)|rdQ(v)]1/r. Thus, given a sample {Dt}n
t=1
and h(·; G), we have ||h(·; G)||Qαn ,2 =
[ 1∑n
t=1 αn,t
∑
t αn,th(Dt; G)2
]1/2
.
In the stationary case, we define the restricted function class Hn = {h1:n : h1:n ∈ H ×
H × · · · × H, h1 = h2 = · · · = hn} and the envelope function Hn = (H1, H2, · · · , Hn)′.
Furthermore, let Q denote the class of all discrete probability measures on the domain of
the random vector Dt = {Yt, Wt, Xt−1}. Recall for a n-dimensional vector v = {v1, . . . , vn},
its l2−norm is denoted by |v|2
def
= (∑n
i=1 v2
i )1/2. Then, for any αn ∈ Rn
+ and  ̃αn,t = √αn,t
√∑
t αn,t
,
we have
N (δ| ̃αn ◦ Hn|2,  ̃αn ◦ Hn, |.|2) = N (δ||H||Qαn ,2, H, ||.||Qαn ,2) ≤ sup
Q∈Q
N (δ||H||Q,2, H, ||.||Q,2).
In light of this relationship in the stationary case, we generalize the setup. Let K to be a
subset of {1, · · · , n}, and its dimension is K = |K|. Let αn,K denote the K dimensional sub-
vector of αn corresponding to the index set K. Recall that Ht denote the envelope function
of Ht, the functional class corresponding to {ht(., G), G ∈ G}, and Hn = H1 × H2 × · · · × Hn.
Then, for the subset K, we similarly define Hn,K as the corresponding functional class, and
the vector of its envelope functions as Hn,K .
Let consider the following assumption: for any fixed K, the covering number can effectively
be reduced to K dimension, i.e.,
N (δ| ̃αn ◦ Hn|2,  ̃αn ◦ Hn, |.|2) ≤ max
K⊆{1:n} N (δ| ̃αn,K ◦ Hn,K |2,  ̃αn,K ◦ Hn,K, |.|2),
≤ max
K⊆{1:n}
∏
t∈K
N (δ| ̃αn,t ◦ Ht|2,  ̃αn,t ◦ Ht, |.|2),
≤ sup
Q
max
t∈K max
K⊆{1:n} N (δ∥Ht∥Q,2, Ht, ∥.∥Q,2)K .
57
The first inequality of (39) in Assumption 3.8 holds by setting K = |K| = 1. Under this as-
sumption, it suffices to examine the one-dimensional covering number N (δ∥Ht∥Q,2, Ht, ∥.∥Q,2).
To provide an example for the second inequality of (39), we let 1(Xt−1 ∈ G) = 1(X⊤
t−1θ ≤ 0)
for some θ ∈ Θ, where Θ is a compact set in Rd. Without loss of generality we assume
that Θ is the unit ball in Rd, i.e., for all θ ∈ Θ: |θ|2 ≤ 1. For w = 0 and 1, define
St,w
def
= Yt(w)1(Wt = w)/ Pr(Wt = w|Xt−1), where Yt(w) is the abbreviation of Yt(Wt−1, w).
Under Assumption 3.7, |Yt(1)|, |Yt(0)| ≤ M/2, so we have ∥Ht∥Q,r ≤ M + M/κ def.
= M ′, and
hθ
t = E(Yt(1)1(X⊤
t−1θ ≤ 0)|Xt−1) + E(Yt(0)1(X⊤
t−1θ > 0)|Xt−1)
−St,11(X⊤
t−1θ ≤ 0) − St,01(X⊤
t−1θ > 0).
The corresponding functional class can be written as
Ht = {h : (yt, wt, xt−1) → f θ
1,1 + f θ
1,0 + f θ
0,1 + f θ
0,0, θ ∈ Θ},
where f θ
1,1 (resp. f θ
1,0, f θ
0,1, and f θ
0,0) corresponds to E(Yt(1)1(X⊤
t−1θ ≤ 0)|Xt−1) (resp.
E(Yt(0)1(X⊤
t−1θ > 0)|Xt−1), −St,11(X⊤
t−1θ ≤ 0), −St,01(X⊤
t−1θ > 0)). Denote the correspond-
ing functional class as F1,1 (resp. F1,0, F0,1, and F0,0). For all finitely discrete norms Q and
any positive ε, we know that
sup
Q
N (ε, Ht, ∥.∥Q,r) ≤ sup
Q
N (ε/4, F1,1, ∥.∥Q,r)N (ε/4, F1,0, ∥.∥Q,r)N (ε/4, F0,1, ∥.∥Q,r)N (ε/4, F0,0, ∥.∥Q,r).
(83)
We look at the covering number of the respective functional class. According to Lemma
9.8 of Kosorok (2008), the subgraph of the function 1(X⊤
t−1θ ≤ 0) is of VC dimension less
than d + 2 since the class {x ∈ Rd, x⊤θ ≤ 0, θ ∈ Θ} is of VC dimension less than d + 2 (see
the proof of Lemma 9.6 of Kosorok (2008)). Therefore, we have supQ N (ε/4, F0,1, ∥.∥Q,r) ∨
N (ε/4, F0,0, ∥.∥Q,r) ≲ (4/(εM ′))d+2.
Moreover, we impose the following Lipschitz condition on functions f θ
1,1,f θ
1,0: For any dis-
tinct points θ, θ′ ∈ Θ and a positive constant Md, it holds that ||f θ
1,1 − f θ′
1,1||Q,r ≤ Md|θ − θ′|r
(the similar for f θ
1,0). It falls within the type II class defined in Andrews (1994), so according
to the derivation of the (A.2) Andrews (1994) we have
sup
Q
N (εM ′, F1,1, ∥.∥Q,r) ≤ sup
Q
N (εM ′/Md, Θ, ∥.∥Q,r), (84)
where the latter is the covering number of a Euclidean ball with ∥.∥Q,r. Thus, according to
Equation (5.9) in Wainwright (2019), supQ N (εM ′/Md, Θ, ∥.∥Q,r) ≲ (1 + 2Md/εM ′)d. Com-
bining the above results, we have supQ N (εM ′, Ht, ∥.∥Q,r) ≲ (4/(εM ′))2(d+2)(1+2Md/(εM ′))2d.
Finally, after some rearrangement and redefinition of constant terms, we can obtain (39).
58
A.5 Proof of Theorem 3.2
In this proof, we show the concentration of I = 1
T −1
∑T −1
t=1  ̃St(G) + 1
T −1
∑T −1
t=1 St(G). Under
Assumptions 3.8 and 3.13 and with similar arguments as those for Lemma A.4, we have
supG∈G
1
T − 1
T −1∑
t=1
St(G) ≲p M √v/√T − 1. (85)
For 1
T −1
∑T −1
t=1  ̃St(G), we first show
(i) For a finite function class G with |G| =  ̃M < ∞ and under Assumptions 3.10- 3.12,
sup
G∈G
1
T − 1
T −1∑
t=1
 ̃St(G) ≤ cT [log  ̃M 2eγ]1/γ Φφ ̃v ,F
√T − 1 , (86)
with probability 1 − exp(−cγ
T ), where cT is a large enough constant, and Φφ ̃v ,F is defined in
Assumption 3.12.
Then, we extend the above result to obtain Theorem 3.2:
(ii) Let G be a function class with infinite elements, whose complexity is subject to Assump-
tion 3.13. Under Assumptions 3.10- 3.13, we have
sup
G∈G
1
T − 1
T −1∑
t=1
 ̃St(G) ≲p
cT [V log T 2eγ]1/γ Φφ ̃v ,F
√T − 1 .
Proof. By Assumption 3.1 and Assumption 3.11(i), E(St(G)|Ft−2) = E(St(G)|Xt−2). By As-
sumption 3.10, E(St(G)|Xt−2) are continuously differentiable with respect to the underlying
i.i.d. innovations. Denote  ̃εt−l−2 as a point between εt−l−2 and ε∗
t−l−2 such that the following
equation holds.
 ̃St(G) −  ̃S∗
t,l(G)
= E(St(G)|Xt−2) − E(St(G)|X∗
t−2,l)
= ∂ E(St(G)|Xt−2)/∂εt−l−2|εt−l−2= ̃εt−l−2 (εt−l−2 − ε∗
t−l−2)
≤ |Ft,l(Xt−2, εt−l−1)(εt−l−2 − ε∗
t−l−2)|.
Thus, the dependence adjusted norm satisfies θx,q ≤ ∑
l≥0 maxt ∥Ft,l(Xt−2, εt−l−1)(εt−l−2 −
ε∗
t−l−2)∥q, and
Φφ ̃v (  ̃S.(G)) ≤ sup
q≥2
(∑
l≥0
max
t ∥Ft,l(Xt−2, εt−l−1))(εt−l−2 − ε∗
t−l−2)∥q)/q ̃v def
= Φφ ̃v ,F (87)
holds for any G ∈ G. Following Assumption 3.12, we have Φφ ̃v (  ̃S.(G)) < ∞. Recall γ =
59
1/(1 + 2 ̃v), and for a finite G with |G| =  ̃M , the next exponential bound follows by Theorem
3 of Wu and Wu (2016).
Pr(sup
G∈G
T −1∑
t=1
 ̃St(G) ≥ x) ≤  ̃M exp
[
−
(
x
√T − 1Φφ ̃v (  ̃S.(G))
)γ
1
2eγ
]
. (88)
Set x = cT [log  ̃M 2eγ]1/γ Φφ ̃v (  ̃S.(G))√T − 1, where cT is a sufficiently large constant, then
sup
G∈G
1
T − 1
T −1∑
t=1
 ̃St(G) ≲p cT [log  ̃M 2eγ]1/γ Φφ ̃v ,F /√T − 1, (89)
with probability 1 − exp(−cγ
T ).
We now verify (ii), where G is not finite. We define G(1)δ to be the δsupQ∥Fp∥Q,2-net of G.
We denote π(G) as closest component of G in the net G(1)δ . Then,
sup
G
1
T − 1
∑
t
 ̃St(G)
≤ sup
G∈G
1
T − 1
T∑
t=1
(  ̃St(G) −  ̃St(π(G))) + sup
G∈G(1)δ
| 1
T − 1
T −1∑
t=1
(  ̃St(G))|
≤ δsupQ∥Fp,t∥Q,2 + sup
G∈G(1)δ
| 1
T − 1
T −1∑
t=1
(  ̃St(G))|
≲p δsupQ∥Fp,t∥Q,2 + cT [V log(1/δ)4eγ]1/γ Φφ ̃v ,F /√T − 1,
where V and δ following the first ≲p are the constants in the first statement of Assumption
3.13. Φφ ̃v ,F is defined in Assumption 3.12. Finally, by setting δ ≪ √T − 1−1,
sup
G
1
T − 1
∑
t=1
 ̃St(G) ≲p cT [V log T 2eγ]1/γ Φφ ̃v ,F /√T − 1. (90)
60
B Appendix of application
B.1 Time series plots of the raw data
Figure 5. Weekly cases and deaths from 4-2020 to 1-2022
Figure 6. Restriction level and economic condition from 4-2020 to 1-2022
61
Figure 7. Vaccine coverage from 4-2020 to 1-2022
The vaccine coverage is calculated by summing up the coverage rate of each dose.
B.2 Estimated propensity scores
Figure 8. Estimated propensity scores
62
B.3 Policy choices based on increased number of variables
Figure 9. Optimal policies based on
XP
T −1 = (change in casesT −1, restriction stringencyT −1, vaccine coverageT −1
)
In the left panel, the x-axis is the change in deaths at week T − 1, and the y-axis is the stringency of
restrictions at week T − 1; in the right panel, the x-axis is the stringency of restrictions at week T − 1, and
the y-axis is the vaccine coverage at week T − 1.
Figure 10. Optimal policy based on
XP
T −1 = (change in deathsT −1, restriction stringencyT −1, vaccine coverageT −1,
change in casesT −1)
In the left panel, the x-axis is the change in deaths at week T − 1, and the y-axis is the stringency of
restrictions at week T − 1; in the right panel, the x-axis is the vaccine coverage at week T − 1, and the y-axis
is the change in cases at week T − 1.
63
C Link to Markov decision problems
In this section, we show the connection between our T-EWM setup and models of Markov
Decision Processes (MDP). For MDP, we adapt the notation of Kallenberg (2016), an
online lecture notes by Lodewijk Kallenberg (LK hereafter). As described in LK, MDP
are models for making decisions for dependent data. A MDP typically has components
{[pij (a)]i,j , rt
i (a), Wt−1}. In period t, Wt−1 is the state and Wt is the action. The agent
chooses their decision according to a policy (a map from the state Wt−1 to an action a).
They then receive a reward rt
i (a). The reward function depends on the transition probabili-
ties of a Markov process, which are determined by the action a. Thus their action affects the
reward via its effect on the transition probability matrix. The optimal policy is estimated
by optimizing an aggregated reward function. We show a formal link between our EWM
framework and an MDP. In particular, we show that the MDP’s reward function corresponds
to our welfare function, and the optimal mapping between states and actions corresponds to
the EWM policy in our framework.
In the following equations, the left-hand sides are the notation for MDP in LK, and the
right-hand sides are notation for T-EWM from this paper. We consider the model of Section
2.2. For i, j, a ∈ {0, 1}, at time t: First, we link the transition probability with the propensity
score.
pt
ij (a) = P (Wt = j|Wt−1 = i; choosing Wt = a),
The left-hand side is the Markov transition probability between states i and j under policy a.
The right-hand side is a propensity score under policy a: the probability Wt = j, conditional
on Wt−1 = i, given Wt = a. Note that, in this simple model, the state at time t is the
previous treatment Wt−1, and the current policy and the next-period state are both Wt. In
our setting, after time T − 1, the SP implements a deterministic policy, so the probability
only takes values in {0, 1}, i.e.,
pt
ij (a) = 1 if j = a.
pt
ij (a) = 0 if j ̸ = a. (91)
Secondly, we connect the reward function with the expected conditional counterfactual out-
come. We denote the reward associated with action a for state i at time t as
rt
i (a) = E [Yt(a)|Wt−1 = i] , (92)
The left-hand side is the reward in state i under action a. The right-hand side is the
conditional expected counterfactual outcome of Yt(a), (recall a ∈ {0, 1}) conditional on
64
Wt−1 = i.
Thirdly, we link the expected reward function and the expected unconditional counterfac-
tual outcome.
{∑
i
βirt
i (a) = rt(a)
}
= E [Yt(a)] ,
The left-hand side is the expected reward for action a, with βi as the initial probability of
state i. The right-hand side is the unconditional expected counterfactual outcome.
Finally, we show the link between the total expected reward over a finite horizon and the
finite-period welfare function
{
vT :T +1
i (R) := E i,R
[T +1∑
k=T
rk
Xk (Yk)
]}
= E
{
YT (1)pT
i1 (g1(WT −1)) + YT (0)pT
i0 (g1(WT −1))
+ YT +1(1)pT +1
i1 (g2(WT )) + YT +1(0)pT +1
i0 (g2(WT )) |WT −1 = i
}
= E {YT (1)g1(WT −1) + YT (0) [1 − g1(WT −1)] |WT −1 = i}
+ E {YT +1(1)g2 (WT ) + YT +1(0) [1 − g2 (WT )] |WT = g1(i)} , (93)
The left-hand side is the total expected reward over the planning horizon from T to T + 1
under the policy R = (g1, g2), with the initial state i. The last equality follows from (91)
and the exclusion condition.
With these connections established, we can regard EMW as an MDP with a finite period
reward and a non-stationary solution. According to LK, in this case the policy R is usually
obtained using a dynamic programming algorithm.
D The relationship between the conditional and un-
conditional cases
In this section, we present further examples to illustrate that G∗
FB ∈ G is a sufficient but
not necessary condition for equivalence between the unconditional and conditional problems.
Finally, we extend Example 4.1 to show how Assumption 3.4 ensures this equivalence.
65

excess returns tend to be high on the day of FOMC announcements.
\cite{cieslak2019stock} show that the excess returns
in even weeks after the FOMC announcement are significantly higher
than those in odd weeks.

In this section, we study the optimal policy region for a fictional
monetary policy target: excess stock returns. Excess returns instantly reflect market confidence and are highly correlated with economic indicators. We attempt to address the following questions:  if the objective of a fictional decision maker is to increase stock
market returns, when should they decrease the target interest rate?


We take treatment variables and covariates that predict the treatment from the monthly dataset of \cite{angrist2018semiparametric}(AJK hereafter).\footnote{We are
	grateful to Joshua Angrist, who shared the data and the replication codes. It is now also available at his website
https://economics.mit.edu/faculty/angrist/data1/data}
Our treatment variable is the change in the Federal target rate.  We define the treatment $W_t=1$ to correspond to a decrease in
the federal target rate, and set $W_t=0$ otherwise. We use the same specification for the propensity score function as AJK, which is
constructed to be a Taylor-type monetary policy rule. The covariates for the propensity score function include
market expectations, which are given by an adjusted difference between the futures contract price and the current target rate (See AJK
and their supplemental data Appendix for more details of this measure), inflation, changes of unemployement rates, lags of
inflation, lagged changes in unemployement rates, the current target rate, the last change of FOMC, a dummy variable
indicating months with a scheduled FOMC meeting, an interaction term of the last change of FOMC and the dummy for FOMC, a
scale factor indicating the part of a month in which a FOMC meeting is scheduled, a set of monthly dummies, and dummies for Y2K and the September 11 attacks. The data runs from August 1989 to July 2005 and contains 128 FOMC meetings.

We use the five-day cumulative excess stock returns in the week of FOMC meetings (Week-0) as our outcome variable. This data is taken from the dataset of \cite{cieslak2019stock}.\footnote{We grateful to Anna Cieslak, Adair Morse and
Annette Vissing-Jorgensen for posting the data and the replication codes at
https://onlinelibrary.wiley.com/doi/abs/10.1111/jofi.12818} The five-day cumulative excess return is defined as the
difference between the cumulative stock return and the five-day cumulative return on 30-day Treasury bills.  We select the
excess returns on the days of the 128 FOMC meetings.

We consider the quadrant treatment rules described in \eqref{eq:quadrant  treatment}.
In this case, we assume that the decision-maker makes decisions based on whether the inflation rate and market
expectations exceed certain bounds.


\begin{figure}[H]
	\centering
	\begin{minipage}{0.35\textwidth} %trying to force figs apart
		\includegraphics[width=70mm]{pictures/ex5_me_in}
		\centering
		(a)  Five-day cumulative excess return
		% difficult text to linebreak nicely?
	\end{minipage}
	\hfil
	\begin{minipage}{0.35\textwidth}
		\includegraphics[width=70mm]{pictures/lagged_ex5_me_in}
		\centering
		(b) Lagged Five-days cumulative excess return
		
	\end{minipage}
	\caption{\label{quadrant}Treatment rules from the quadrant class conditioning on market expectation and inflation rate.}
\end{figure}

Figure \ref{quadrant} shows the quadrant treatment rules selected by T-EWM. The shaded region corresponds to the area in which the policy maker should set $W_t=1$ (i.e. cut the interest rate).  The left panel, (a), shows that a decision maker aiming to maximize the week-0 cumulative excess return should decrease the target rate
if \textit{market expectation} $\geq$  -0.2845 and \textit{inflation} $\geq$ 0.1337. A cut in the interest rate is more likely to increase stock market values if inflation is high, and the market expects an increase in the target rate.

The right panel of Figure \ref{quadrant} illustrates the treatment rule for the lag-1 case. The shaded region is consistent with the following mechanism. Suppose that the inflation rate reflects the expectation of the general public, while market expectations reflect the expectations of professional traders who collectively determine the prices of futures. Panel (b) shows that experienced traders react to monetary policy faster than the general public: excess stock returns at the
beginning of the next FOMC cycle are more likely to increase following a cut in the target rate in the current period if the inflation rate is high but experienced traders anticipated the decrease in the target rate.



==> App_ass_short.tex <==
\subsection{On Assumptions \ref{cover1} to \ref{D.4}} \label{sec:ass_of_Sec3}

In this section, we verify the theoretical hyper Assumptions \ref{cover1} to \ref{D.4} in Section \ref{continuous} using the setup Example \ref{example_q1_Markov}.
\subsubsection{Notations}
{To avoid the conflict of notations, we use $\eta_t$ to replace the error term $\vps_t$ of the DGP in Exmaple \ref{example_q1_Markov}. Specifically, within this section,  the notations of equation \eqref{eq:Yt} and \eqref{eq:et} are modified to:
\begin{align*}
Y_{t} & =\beta_0 + \beta_{1}W_{t}+\beta_{2}W_{t-1}+\eta_{t}, \,\,\quad\qquad\qquad\qquad\qquad \qquad\qquad \qquad \text{\eqref{eq:Yt}}\\
 \eta_t & \perp (W_t, X_{0:t-1}) \qquad \forall 1 \leq t \leq T-1  \qquad \text{and} \qquad  \eta_T  \perp X_{0:T-1}\qquad \text{\eqref{eq:et}}
 \end{align*}}
First, we study the meanings of the general definitions used in Section \ref{continuous} in the context of Example \ref{example_q1_Markov}. Recall that for the DGP in Example \ref{example_q1_Markov}, $X_t\equiv W_t$. Then, 
\begin{align*} S_{t}(G)&=
Y_{t}(W_{t-1},1)\IF(X_{t-1}\in G)+Y_{t}(W_{t-1},0)\IF(X_{t-1}\notin G)\\
&=\beta_{0}+\beta_{1}\IF(W_{t-1}\in G)+\beta_{2}W_{t-1}+\eta_t,
\end{align*}
where $G\in \mathcal{G}\equiv\left\{ \emptyset,\{0\},\{1\},\{0,1\}\right\}$.
By \eqref{eq:Wt} to \eqref{eq:Vt_2}, 

 Recall that $\mathcal{F}_{t-1}=\sigma(X_{0:t-1})$.
Then, $\E(\eta_t|\mathcal{F}_{t-1})=0$ yields
\begin{align*}
	& \E(S_{t}(G)|\mathcal{F}_{t-1}) 
 %=\E[Y_{t}(W_{t-1},1)|\mathcal{F}_{t-1}]\IF(X_{t-1}\in G)+\E(Y_{t}(W_{t-1},0)|\mathcal{F}_{t-1})\IF(X_{t-1}\notin G)\\
%	& =\E[\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}+\varepsilon_{t}|\mathcal{F}_{t-1}]\IF(X_{t-1}\in G)+\E(\beta_{0}+\beta_{2}W_{t-1}+\varepsilon_{t}|\mathcal{F}_{t-1})\IF(X_{t-1}\notin G)\\
%	& =\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}+[-\beta_{0}-\beta_{2}W_{t-1}-\beta_1+\E(\beta_{0}+\beta_{2}W_{t-1}+\varepsilon_{t}|\mathcal{F}_{t-1})]\IF(X_{t-1}\notin G)\\
	 =\beta_{0}+\beta_{1}\IF(W_{t-1}\in G)+\beta_{2}W_{t-1}.
\end{align*}
Moreover, recall that 
\beaa
		\tilde{S}_{t}(G)&=&\E(S_{t}(G)|\mathcal{F}_{t-2})-\E(S_{t}(G)),\\
		\overline{S}_{t}(G)  &=&\E(S_{t}(G)|\mathcal{F}_{t-1})-\E(S_{t}(G)|\mathcal{F}_{t-2}).
  \eeaa
Thus, $W_{t-1}-\E(W_{t-1}|\mathcal{F}_{t-2})=V_{t-1}$.
Defining the conditional probability $\Pr{_{t-2}}(X_{t-1} \in G) = \E(1(X_{t-1}\in G)|\mathcal{F}_{t-2})$, for Example \ref{example_q1_Markov},
\begin{align*}
\tilde{S}_{t}(G)&=\beta_{1}(\Pr{_{t-2}}(X_{t-1}\in G)-\Pr(X_{t-1}\in G))+\beta_{2}(\E(W_{t-1}|\mathcal{F}_{t-2})-\E(W_{t-1}))\\
	\overline{S}_{t}(G)
		 &=\beta_{1}[1(X_{t-1}\in G)-\Pr{_{t-2}}(X_{t-1}\in G)]+\beta_{2}[W_{t-1}-\E(W_{t-1}|\mathcal{F}_{t-2})].
	\end{align*}
By the fact that $\E(\varepsilon_{t}|\mathcal{F}_{t-2})=0.$
Also we have $ \E(S_{t}(G)|\mathcal{F}_{t-2})=\beta_{0}+\beta_{2}\E(W_{t-1}|\mathcal{F}_{t-2})+\beta_{1}\P_{t-2}(X_{t-1}\in G)$. Denote $G^*$ as the $G$ corresponding to this envelope.
$|\E(\tilde{S}_{t}(G)|\mathcal{F}_{t-2})|$ shall be a function of
$X_{t-2}$ due to the condition that $X_{t}\perp X_{0:t-1}|X_{t-1}$.
Denote this function as $|\E(\tilde{S}_{t}(G)|\mathcal{F}_{t-2})| = m(X_{t-2},G)$.
We have $|\partial\E(\tilde{S}_{t}(G)|\mathcal{F}_{t-2})/\partial\varepsilon_{t-l-1}|=|\partial m(X_{t-2}, G)/(\partial X_{t-2}\partial\eta_{t-l-1})|$.

\subsubsection{Verification of assumptions} 
\begin{itemize}
	\item[i)] (Assumptions \ref{cover1} and \ref{D.4}) We can see that the Assumption 3.8 and 3.13 are of similar fashion, since the subgraph class corresponding to the indicator function and the conditional probability function would both be affected by the complexity of $\mathcal{G}$ in a similar fashion. See Theorem 9.2 in \cite{kosorok2008introduction} and Lemma 9.7 v) as the function $\Pr{_{t-2}}(X_{t-1}\in G))$ is one to one. The covering number of the subgraph class corresponding to $X_{t-1}\in G, G \in \mathcal{G}$ is related to $1(X_{t-1} \in G), G \in \mathcal{G}$.   
	It shall be noted that if the data is stationary, then 
	$$\mathcal{N}(\delta|\tilde{\alpha}_{n}\circ\overline{\tilde{F}}{}_{n}|_{2},\mathbf{\tilde{\alpha}_{n}\circ\tilde{F}_{n},|.|_{2}})\leq\max_{t}\sup_{Q}[\mathcal{N}(\delta\|\tilde{F}_{t}\|_{Q,2},\tilde{\mathcal{S}}_{t},\|.\|_{Q,2})]\lesssim(1/\delta)^{v},$$
	then we can study the covering number for any $t$.
	Thus it boils down to study $$\max_{t}\sup_{Q}[\mathcal{N}(\delta\|\tilde{F}_{t}\|_{Q,2},\tilde{\mathcal{S}}_{t},\|.\|_{Q,2})],$$ and it can be studied in the same fashion as in Lemma A.1 in \cite{kitagawa2018should}.
	This is because that if the data is iid and $\overline{S}_{t}(G)$
	and $\tilde{S}_{t}(G)$ induce the same class of functions.
	$$\ensuremath{\overline{H}_{n}=(H_{1},H_{1},\cdots,H_{1})^{\prime}}.$$
	Otherwise if the data is not stationary, we let $\ensuremath{\mathbf{H_{n}}=\mathcal{\mathcal{H}}_{1}\times\mathcal{\mathcal{H}}_{2}\times\dots\times\mathcal{H}_{n}.}$
	Let $\tilde{\alpha} $ be a vector of $(\alpha_1, \alpha_2,\cdots, \alpha_n)$.Suppose there are two regime with $\ensuremath{\overline{H}_{n}=(H_{1},H_{2},H_{[n/2]},H_{[n/2]+1}\cdots,H_{n})^{\prime}}=(H_{1},H_{1},H_{1},H_{2}\cdots,H_{2})^{\prime}$. $\|\tilde{\alpha} \circ \overline{H}_{n}\|=\sqrt{\alpha_1^2+\cdots+\alpha_{\lfloor n/2\rfloor}^2}\|H_{1}\|+\sqrt{\alpha_{\lfloor n/2\rfloor+1}^2+\cdots+\alpha_{n}^2}\|H_{2}\|.$ 
	
	Then the covering number holds for, $$\mathcal{N}(\delta|\tilde{\alpha}_{n}\circ\overline{\tilde{F}}{}_{n}|_{2},\mathbf{\tilde{\alpha}_{n}\circ\tilde{F}_{n},|.|_{2}})\leq\max_{t}\sup_{Q}[\mathcal{N}(\delta\|\tilde{F}_{t}\|_{Q,2},\tilde{\mathcal{S}}_{t},\|.\|_{Q,2})]^2\lesssim(1/\delta)^{2v}.$$ 
 {\blue [In this case the c in the main text is 2]}
	
	
	
	
	\item[ii)] (Assumption \ref{norm}) Namely we need to prove that,
	there exists a positive constant $L>0$ such that $\Pr(\sigma_{n}(f,g)/\rho_{2,n}(f,g)>L)\to0$
	as $n\to\infty$. Also, $$\Pr(\left(n^{-1}\sum_{t}\E[(f_{t}-g_{t})^{2}|\mathcal{F}_{t-2}]\right)^{1/2}/\rho_{2,n}(f,g)>L)\to_{n\to\infty}0,$$
	
	where $\rho_{2,n}(f,g)=(n^{-1}\sum_{t}|f_{t}-g_{t}|^{2})^{1/2}$ and $\sigma_{n}(f,g)=\left(n^{-1}\sum_{t}\E[(f_{t}-g_{t})^{2}|\mathcal{F}_{t-1}]\right)^{1/2}$.
	Recall that we have 
	\begin{align*}\widehat{\mathcal{W}}_{t}(G) & =\frac{Y_{t}W_{t}}{e_{t}(X_{t-1})}1(X_{t-1}\in G)+\frac{Y_{t}(1-W_{t})}{1-e_{t}(X_{t-1})}1(X_{t-1}\notin G),\\
		\bar{\mathcal{W}}_{t}(G) & =\mathsf{E}\left\{ Y_{t}(W_{t-1},1)1(X_{t-1}\in G)+Y_{t}(W_{t-1},0)1(X_{t-1}\notin G)|\mathcal{F}_{t-1}\right\} .
	\end{align*}
	
	
	We let
	\begin{align*}
		\widehat{\mathcal{W}}_{t}(G)-\bar{\mathcal{W}}_{t}(G) & =\frac{Y_{t}W_{t}}{e_{t}(X_{t-1})}1(X_{t-1}\in G)+\frac{Y_{t}(1-W_{t})}{1-e_{t}(X_{t-1})}1(X_{t-1}\notin G)\\
		& -\mathsf{E}\left\{ Y_{t}(W_{t-1},1)1(X_{t-1}\in G)+Y_{t}(W_{t-1},0)1(X_{t-1}\notin G)|\mathcal{F}_{t-1}\right\}.
	\end{align*}
	
	Thus for a specific $G$ corresponding to $f_{t}$, we have
	\begin{align*}
		f_{t} & =[\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\in G)/e_{t}(X_{t-1})\\
		&+[\beta_{0}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\notin G)/(1-e_{t}(X_{t-1})) -[\beta_{1}1(X_{t-1}\in G)+\beta_{0}+\beta_{2}W_{t-1}].
	\end{align*}
	
	Thus for $G'$ corresponding to $g_{t}$, we have that,
	\begin{align*}
		g_{t}-f_{t} & =[\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\in G)/e_{t}(X_{t-1})\\
		& +[\beta_{0}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\notin G)/(1-e_{t}(X_{t-1}))-\beta_{1}1(X_{t-1}\in G)\\
		& -[\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\in G')/e_{t}(X_{t-1})\\
		& -[\beta_{0}+\beta_{2}W_{t-1}+\varepsilon_{t}]1(X_{t-1}\notin G')/(1-e_{t}(X_{t-1}))+\beta_{1}1(X_{t-1}\in G').
	\end{align*}
	%Denote two sets $A$ and $B$ and $A \Delta B=(A \backslash B) \cup(B \backslash A)$.
	Let
	\begin{align*}
		c_{t-1} & =[\beta_{0}+\beta_{1}+\beta_{2}W_{t-1}]1(X_{t-1}\in G \backslash G')/e_{t}(X_{t-1})+[\beta_{0}+\beta_{2}W_{t-1}]\\
		&1(X_{t-1}\not \in G \backslash G')/(1-e_{t}(X_{t-1}))
		-\beta_{1}1(X_{t-1}\in G\backslash G'),\\
		d_{t-1} & =1(X_{t-1}\in G\backslash  G')/e_{t}(X_{t-1})+1(X_{t-1} \not \in G \backslash G')/(1-e_{t}(X_{t-1})).
	\end{align*}
	
	Then $\sigma_{n}(f,g)$ only concerns $\E\{[c_{t-1}+\varepsilon_{t}d_{t-1}]^{2}|\mathcal{F}_{t-1}\}=c_{t-1}^{2}+\E(\varepsilon_{t}^{2}|\mathcal{F}_{t-1})d_{t-1}^{2}$.
	
	Define a positive constant $c$.
	Under conditional homoscedascity we have $\E(\varepsilon_{t}^{2}|\mathcal{F}_{t-1})=c$, thus $\Pr(\sigma_{n}(f,g)/\rho_{2,n}(f,g)>L)\to0$ follows naturally
	with decay dependence of the process, as $\rho_{2,n}(f,g)$ $\sigma_{n}(f,g)$ all approach to  $\mbox{lim}_{T\to\infty}\E\rho_{2,n}(f,g)$ in the probability limit. Similar for $n^{-1}\sum_{t}\E[(f_{t}-g_{t})^{2}|\mathcal{F}_{t-2}]=\sum_{t}[\E(c_{t-1}^{2}|\mathcal{F}_{t-2})+c\E(d_{t-1}^{2}|\mathcal{F}_{t-2})].$
	
	\item[iii)] (Assumption \ref{D.1})
	{\blue This assumption is satisfied by iterating \eqref{eq:Wt}, leading to 
$W_{t}=g(V_t,V_{t-1},\cdots):=\frac{1-q}{1-\lambda}+\sum_{l\geq 0}\lambda^{l}V_{t-l}.$} It should be noted that the notation $\varepsilon_t$ used in Assumption \ref{D.1} corresponds to $V_t$ in Example \ref{example_q1_Markov} .
{\color{red}$W_t = \IF(\sum_{\ell}a_{\ell}\eta_{t-\ell}>0)$}

	\item[iv)] (Assumption \ref{D.2})
 Since there is no additional regressor $Z_t$ in Example \ref{example_q1_Markov}, part (i) of this assumption holds trivially. For part (ii), the DGP of Example \ref{example_q1_Markov} suggests that $E(\tilde{S}_{t}(G)|\mathcal{F}_{t-2})=p$ in the case $W_{t-2}=1$ and $E(\tilde{S}_{t}(G)|\mathcal{F}_{t-2})=1-q$ in the case $W_{t-2}=0$, thus
	The envelope function of $S_{t}(G) -\E(S_{t}(G)|\mathcal{F}_{t-2})$ is $\sup_{G \in \mathcal{G}}|\beta_{1}(1(X_{t-1}\in G)-\P_{t-2}(X_{t-1}\in G))|+|\beta_{2}(W_{t-1}-\E(W_{t-1}|\mathcal{F}_{t-2}))|.$ 
%	The envelop of $|\partial m(X_{t-2}, G)/$ $(\partial X_{t-2}\partial\eta_{t-l-1})|$ follows from the same argument.
	%Denote $G^*$ as the solution maximizing $|\partial m(X_{t-2}, G)/(\partial X_{t-2}\partial\eta_{t-l-1})|$. We have 
	%$F_{t,l}(X_{t-2},\eta_{t-l-1})=|\partial m(X_{t-2},G^*)/$ $\partial X_{t-2}\partial X_{t-2}/\partial\eta_{t-l-1}|$.
	\item[v)] (Assumption \ref{D.3})
	It is not hard to imagine that Assumption \ref{D.3} holds true with moment
	restrictions on the shocks $\eta_{t}$ and boundedness or moment property of the derivative function $\partial m(X_{t-2}, G)/\partial X_{t-2}$. 
\end{itemize}


==> App_proof_Sec6_lb.tex <==


\subsubsection{Proof of Theorem \ref{th:lower_bound}} \label{sec: proof_lower}
\begin{proof}
	We can assume a specific data generating process. Let $Y_{t}(W_{0:t})=Y_{t}(W_{t})$ with $W_{t}$ i.i.d. over time with $\P(W_{t}=1)=1/2$ and $\P(W_{t}=0)=1/2$. Let $v$ be an integer. Let $\mathbf{b}=(b_{1},b_{2},\cdots,b_{v})$ be the class of models indexed by a $v$ dimensional $0,1$
	vector, which will have $2^{v}$
	elements. $j = 1, \cdots, v$ corresponds to $j$  different partitions of $X_t$ related to the set $G_j$.
	 Next, we assume that $Y_{t}(1)$ has a binary distribution, with  a positive constant $0<r< 1/2$,
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2+r \quad \text{if} \quad b_j = 1 , X_{t-1}\in G_j ,\\
			-1/2, & \text{with probability}\ 1/2-r\quad \text{if} \quad b_j = 1, X_{t-1} \in G_j  .
		\end{cases}
	\end{equation}
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 1 , X_{t-1}\not\in G_j ,\\
			-1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 1, X_{t-1} \not\in G_j  .
		\end{cases}
	\end{equation}
	Otherwise,
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2 \quad \text{if} \quad b_j = 0 , X_{t-1}\not \in G_j, \\
			-1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 0, X_{t-1}\not \in G_j  .
		\end{cases}
	\end{equation}
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2-r \quad \text{if} \quad b_j = 0 , X_{t-1} \in G_j, \\
			-1/2, & \text{with probability}\ 1/2+r\quad \text{if} \quad b_j = 0, X_{t-1}\in G_j  .
		\end{cases}
	\end{equation}
	
	%
	%with $Y_{t}(1)=1/2$ with probability $1/2+r$ and $Y_{t}(1) = -1/2$ with
	%probability $1/2-r$ for a positive constant $0<r< 1/2$, if $b_{j}=1$.
	%And $Y_{t}(1)=1/2$ with probability $1/2-r$ and $Y_{t}(1)$ with
	%probability $1/2+r$ for a positive constant $r$, if $b_{j}=0$.
	
	and $Y_{t}(0)=0$ if $W_{t}=0$. Let $X_{t}$ be a stationary Markovian process of
	order one. There exists $G_{j}$ ($j=1,\cdots,v$), such that $X_{t}\in G_{j}$
	corresponds to $b_{j}$ and $\Pr(X_{t}\in G_{j})>0$ for all $j$.
	$\cup_{j}G_{j}=G$ is contained in the compact set from which $X_{t}$ takes its value. Thus $\Pr(Y_{t}(1)=1/2|X_{t-1}\in G_{j},b_{j}=1)= 1/2+ r$. We also
	assume that $X_t$ only causes $Y_t(.)$ via $X_{t-1}$, not directly.
	There exists a compact support of $x_{t-1:t}$ containing $G_j$ and $G$, denoted as $B_x$.
	%Assume that $\int_{x_{t-1:t}\in B_x}p(x_{t}|x_{t-1})dx_{t-1}dx_t>\underline{p}$, for a strictly positive function $\underline{p}$ with
%	any $x \in G$.
We abbreviate $Y_{0:T}(.)$ to $Y_{0:T}$. As $\hat{G}$
	is estimated based on the whole sample $(Y_{0:T},W_{0:T})$, we denote $g_{T}(i,X_{0:T},Y_{0:T})=\IF(X_{t-1}\in\hat{G},X_{t-1}\in
	G_{i})$
	and $f_{\mathbf{b}}(i)=\IF(X_{t-1}\in G_{i},b_{i}=1)$, $\IF(X_{t-1}\in\hat{G}\Delta
	G^{*}(\mathbf{b}))=\sum_{i}\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))$.
	We assume $\mathbf{b}$ is uniformly distributed over $2^{v}$
	elements. Moreover, $\E(Y_t(1)|b_j = 1,X_{t-1} \in G_j) =
	1/2((1/2+r)-(1/2-r)) = r$. Then,
	\begin{eqnarray*}
		& & \mathcal{W}_T(G^{*}(\mathbf{b}))-\mathcal{W}_T(\hat{G}),\\
		& \geq & r\E(\IF(X_{t-1}\in\hat{G}\Delta G^{*}(\mathbf{b}))),\quad\quad\text{where }\widehat{G}\Delta G^{*}(\mathbf{b})=(\hat{G}\cap
		G^{*}(\mathbf{b})^{c})\cup(G^{*}(\mathbf{b})\cap\hat{G}^{c}),\\
		& \geq & \frac{r}{v}\sum_{i=1}^{v}\E\{\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))\}.
	\end{eqnarray*}
	We let $y_{0:T}$ denote any particular realized path of $Y_{0:T}(w_{0:T})$.
	The likelihood of the model given one $\mathbf{b}$ can be written
	as
	\begin{equation}
		\P_{\mathbf{b}}(x_{0},x_{1},x_{2},\cdots,x_{T},y_{0},y_{1},y_{2},\cdots,y_{T},w_{0:T})=\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}p(x_{0},y_{0},w_{0}),
	\end{equation}
	where $\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})$ is the conditional density of $y_t$ on $x_{t-1},w_t$ and $\mathbf{b}$.
	We let\\ $\E\{\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))\}=E_{i}$.
	
	We proceed to bound the value of $E_i$. Let $\P_{b_{i+}}(y_{t}|x_{t-1})$ denote
	the probability conditional on $b_{i}=1$, and $\P_{b_{i-}}(y_{t}|x_{t-1})$
	denote the probability conditional on $b_{i}=0$.
	We let
	{\small
		$$p_{+}(x_{0:T},y_{0:T})\defeq [\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{b_{i+}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\},
		p(x_{0},y_{0},w_{0})],$$ and
		$$p_{-}(x_{0:T},y_{0:T})\defeq [\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{b_{i-}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}
		p(x_{0},y_{0},w_{0})].$$}
	
	Then we have,
	\begin{eqnarray*}
		&  & E_{i}=2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}\IF(g_{T}(i,x_{0:T},y_{0:T})=1-f_{\mathbf{b}}(i))\\
		&  & \Pi_{t=0}^{T-1}\{p(x_{t}|x_{t-1})\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}p(x_{0},y_{0},w_{0})dx_{0:T},\\
		& \geq &
		2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}1/2[\IF(g_{T}(i,x_{0:T},y_{0:T})=1)p_{+}(x_{0:T},y_{0:T})\\
		&  &
		+\IF(g_{T}(i,x_{0:T},y_{0:T})=0)p_{-}(x_{0:T},y_{0:T})]dx_{0:T},\\
		& \geq &
		2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}(1/2\{\IF(g_{T}(i,x_{0:T},y_{0:T})=1)+\IF(g_{T}(i,x_{0:T},y_{0:T})=0)\}\nonumber\\
		&  & \min[p_{+}(x_{0:T},y_{0:T}),p_{-}(x_{0:T},y_{0:T})])dx_{0:T}.
	\end{eqnarray*}
There exists a sequence of $x_{t,min,i}\in G_i$ ($t=1:T-1$) such that the following lower bound holds,
	{\small
		\begin{eqnarray*}
			& \geq &
			2^{-(v+1)}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}\min[p_{+}(x_{0:T},y_{0:T}),p_{-}(x_{0:T},y_{0:T})]dx_{0:T},\\
			& \geq &
			2^{-(v+1)}\sum_{\mathbf{b}}(\sum_{y_{0:T},w_{0:T}}\int_{x_{0:T}}[p_{+}(x_{0:T},y_{0:T})p_{-}(x_{0:T},y_{0:T})]^{1/2}dx_{0:T})^{2},\\
			& \geq &
			2^{-(v+2)}\sum_{\mathbf{b}}p_{0}(\sum_{y_{t},w_t}\int_{x_t}\P(w_{t})p(x_t|x_{t-1,min,i})\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1,min,i},w_{t})\P_{b_{i+}}(y_{t}|x_{t-1,min,i},w_{t})}dx_{t})^{2(T-1)},\nonumber
	\end{eqnarray*}}
	where the second to last line is due to the LeCam's Inequality: for any positive sequence of $a_i$ and $b_i$,
	\beq
	\sum_i \min(a_i,b_i)\geq 1/2(\sum_i\sqrt{a_i b_i})^2.
	\eeq
	The last line follows from $p(x_{0},y_{0},w_{0})\geq p_{0}$ for any $x_{t-1}\in G$, which holds as $\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1})\P_{b_{i+}}(y_{t}|x_{t-1})}$ takes the value $\sqrt{1/4-r^2}$ only for  $x_{t-1}\in G_i$ and has value $1/2 $ otherwise.
	%
%	Now we assume $	\int_{ x_{t-1}\in \times G} p(x_{t}|x_{t-1}) dx_{t-1}dx_t\geq\underline{p}> 0$.
	
	
	For $r\geq 0$,
	\begin{eqnarray*}
		&  &
		\sum_{y_{t}\in\{1/2,-1/2,0\},w_{t}\in\{0,1\}}\int_{x_t}\P(w_{t})p(x_t|x_{t-1,min,i})\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1,min,i})\P_{b_{i+}}(y_{t}|x_{t-1,min,i})}dx_{t}\\
		& \geq & \min\{1/2\bigg(\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\{1/2+1/2\}+2\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\sqrt{1/4-r^{2}}\bigg),\\
				&&1/2\bigg(\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}+ \int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\bigg)\}\\
& \geq & (1/2+1/2\sqrt{1-4r^{2}}).
%		& \geq & (1/2\underline{p}_1+1/2\underline{p}_2\sqrt{1-4r^{2}}+1/2\underline{p}_1  +1/2 \underline{p}_2),
	\end{eqnarray*}
%	where we assume that $\int_{x_{t}}\int_{x_{t-1}\not\in
%			G_{i}}p(x_t|x_{t-1})dx_{t-1:t}\geq \underline{p}_1>0$ and $\int_{x_{t}}\int_{x_{t-1}\in G_i}p(x_t|x_{t-1})dx_{t-1:t} \geq  \underline{p}_2>0$, and $\underline{p} = \underline{p}_1 + \underline{p}_2$. It is not hard to see that $\underline{p} \geq 1$.
	
	Thus, as $\sqrt{1-4r^{2}}\geq-4r^{2}+1$, we have
	\begin{eqnarray*}
		E_{i}\geq p_{0}(1-2r^{2})^{2(T-1)}.
	\end{eqnarray*}

So 
\begin{eqnarray*}
W_T(G^{*}(\mathbf{b}))-W_T(\hat{G})\geq (r/v) p_{0}(1-2r^{2})^{2(T-1)}.
\end{eqnarray*}
We maximize the right hand side with respect to $r$. Take logs to obtain, $ \log(r)+\log(p_{0}/v)+2(T-1)\log(1-2r^{2})$.
The first derivative is $r^{-1}+ 2(T-1)(1-2r^2)^{-1} (-4r)=0$. $r$ is thus of order $\sqrt{T-1}^{-1}$.

	
	We take $r=\sqrt{v/(2(T-1))}$, then $E_{i}\geq p_{0}(1-v/(T-1))^{2(T-1)}\geq
	p_{0}\{\exp\{-(v/(T-1))/(1-\frac{v}{T-1})\}\}^{2(T-1)}$, so $r\sum_{i=1}^{v}E_{i}\geq\sqrt{v/(2(T-1))}\exp(-1)$.
\end{proof}



==> App_proof_Sec6_lb_old.tex <==


\subsection{Proof of Theorem \ref{th:lower_bound}} \label{sec: proof_lower}
\begin{proof}
	Since we know that, for any subset of $\mathcal{P}(M,\kappa)$ denoted as $\mathcal{P}'(M,\kappa)$,
	\begin{eqnarray*}
		&&\inf_{\hat{G}}\underset{P\in\mathcal{P}(M,\kappa)}{\text{sup}}\{W_T(G^{*})-W_T(\hat{G})\}\geq\sqrt{v/(T-1)}\exp(-1),\\
		&&\inf_{\hat{G}}\underset{P\in\mathcal{P}'(M,\kappa)}{\text{sup}}\{W_T(G^{*})-W_T(\hat{G})\}\geq\sqrt{v/(T-1)}\exp(-1).
	\end{eqnarray*}
		
	Therefore we can work with a specific data generating process. Let us assume that  $Y_{t}(W_{0:t})=Y_{t}(W_{t})$, and $W_{t}$ are
	iid over time with $\P(W_{t}=1)=1/2$ and $\P(W_{t}=0)=1/2$. Let $v$ be an integer.
	We denote the class of models indexed by a $v$ dimensional $0,1$
	vector $\mathbf{b}=(b_{1},b_{2},\cdots,b_{v})$, which make $2^{v}$
	elements.
	Next we assume that $Y_{t}(1)$ has a binary distribution, with  a positive constant $0<r< 1/2$,
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2+r \quad \text{if} \quad b_j = 1 , X_{t-1}\in G_j ,\\
			-1/2, & \text{with probability}\ 1/2-r\quad \text{if} \quad b_j = 1, X_{t-1} \in G_j  .
		\end{cases}
	\end{equation}
	
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 1 , X_{t-1}\not\in G_j ,\\
			-1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 1, X_{t-1} \not\in G_j  .
		\end{cases}
	\end{equation}
	Otherwise,
	
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2 \quad \text{if} \quad b_j = 0 , X_{t-1}\not \in G_j, \\
			-1/2, & \text{with probability}\ 1/2\quad \text{if} \quad b_j = 0, X_{t-1}\not \in G_j  .
		\end{cases}
	\end{equation}
	\begin{equation}
		Y_{t}(1)=
		\begin{cases}
			1/2, & \text{with probability}\ 1/2-r \quad \text{if} \quad b_j = 0 , X_{t-1} \in G_j, \\
			-1/2, & \text{with probability}\ 1/2+r\quad \text{if} \quad b_j = 0, X_{t-1}\in G_j  .
		\end{cases}
	\end{equation}
	
	%
	%with $Y_{t}(1)=1/2$ with probability $1/2+r$ and $Y_{t}(1) = -1/2$ with
	%probability $1/2-r$ for a positive constant $0<r< 1/2$, if $b_{j}=1$.
	%And $Y_{t}(1)=1/2$ with probability $1/2-r$ and $Y_{t}(1)$ with
	%probability $1/2+r$ for a positive constant $r$, if $b_{j}=0$.
	
	Also $Y_{t}(0)=0$ if $W_{t}=0$. Let $X_{t}$ be a stationary Markovian process of
	order one. There are $G_{j}$ ($j=1,\cdots,v$), such that $X_{t}\in G_{j}$
	corresponds to $b_{j}=1$ and $\P(X_{t}\in G_{j})>0$ for all $j$.
	$\cup_{j}G_{j}=G$ is a compact set where $X_{t}$ takes on value. Thus $\P(Y_{t}(1)=1/2|X_{t-1}\in G_{j},b_{j}=1)= 1/2+ r$. We also
	assume that $X_t$ does not directly cause $Y_t(.)$ but only via $X_{t-1}$.
	There exists a compact support of $x_{t-1:t}$ containing $G_j$ and $G$, denoted as $B_x$.
	%Assume that $\int_{x_{t-1:t}\in B_x}p(x_{t}|x_{t-1})dx_{t-1}dx_t>\underline{p}$, for a strictly positive function $\underline{p}$ with
%	any $x \in G$.
We abbreviate $Y_{0:T}(.)$ to $Y_{0:T}$. As $\hat{G}$
	is estimated based on the whole sample $(Y_{0:T},W_{0:T})$, we denote $g_{T}(i,X_{0:T},Y_{0:T})=\IF(X_{t-1}\in\hat{G},X_{t-1}\in
	G_{i})$
	and $f_{\mathbf{b}}(i)=\IF(X_{t-1}\in G_{i},b_{i}=1)$, $\IF(X_{t-1}\in\hat{G}\Delta
	G^{*}(\mathbf{b}))=\sum_{i}\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))$.
	We shall assume $\mathbf{b}$ to be uniformly distributed over $2^{v}$
	elements. Moreover, $\E(Y_t(1)|b_j = 1,X_{t-1} \in G_j) =
	1/2((1/2+r)-(1/2-r)) = r$, we have that,
	\begin{eqnarray*}
		& & W_T(G^{*}(\mathbf{b}))-W_T(\hat{G}),\\
		& \geq & \frac{r}{v}\E(\IF(X_{t-1}\in\hat{G}\Delta G^{*}(\mathbf{b}))),\quad\quad\widehat{G}\Delta G^{*}(\mathbf{b})=(\hat{G}\cap
		G^{*}(\mathbf{b})^{c})\cup(G^{*}(\mathbf{b})\cap\hat{G}^{c}),\\
		& \geq & \frac{r}{v}\sum_{i=1}^{v}\E\{\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))\}.
	\end{eqnarray*}
	We let $y_{0:T}$ denote any particular realized path of $Y_{0:T}(w_{0:T})$.
	The likelihood of the model give one $\mathbf{b}$ can be written
	as
	\begin{equation}
		\P_{\mathbf{b}}(x_{0},x_{1},x_{2},\cdots,x_{T},y_{0},y_{1},y_{2},\cdots,y_{T},w_{0:T})=\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}p(x_{0},y_{0},w_{0}),
	\end{equation}
	where $\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})$ is the conditional density of $y_t$ on $x_{t-1},w_t$ and $\mathbf{b}$.
	We denote\\ $\E\{\IF(g_{T}(i,X_{0:T},Y_{0:T})=1-f_{\mathbf{b}}(i))\}=E_{i}$.
	
	We shall proceed to bound the value of $E_i$. We denote $\P_{b_{i+}}(y_{t}|x_{t-1})$ as
	the probability conditioning on $b_{i}=1$, and $\P_{b_{i-}}(y_{t}|x_{t-1})$
	as the probability with $b_{i}=0$.
	We let
	{\small
		$$p_{+}(x_{0:T},y_{0:T})\defeq [\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{b_{i+}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\},
		p(x_{0},y_{0},w_{0})],$$ and
		$$p_{-}(x_{0:T},y_{0:T})\defeq [\Pi_{t=1}^{T-1}\{p(x_{t}|x_{t-1})\P_{b_{i-}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}
		p(x_{0},y_{0},w_{0})].$$}
	
	Then we have,
	\begin{eqnarray*}
		&  & E_{i}=2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}\IF(g_{T}(i,x_{0:T},y_{0:T})=1-f_{\mathbf{b}}(i))\\
		&  & \Pi_{t=0}^{T-1}\{p(x_{t}|x_{t-1})\P_{\mathbf{b}}(y_{t}|x_{t-1},w_{t})\P(w_{t})\}p(x_{0},y_{0},w_{0})dx_{0:T},\\
		& \geq &
		2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}1/2[\IF(g_{T}(i,x_{0:T},y_{0:T})=1)p_{+}(x_{0:T},y_{0:T})\\
		&  &
		+\IF(g_{T}(i,x_{0:T},y_{0:T})=0)p_{-}(x_{0:T},y_{0:T})]dx_{0:T},\\
		& \geq &
		2^{-v}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}(1/2\{\IF(g_{T}(i,x_{0:T},y_{0:T})=1)+\IF(g_{T}(i,x_{0:T},y_{0:T})=0)\}\nonumber\\
		&  & \min[p_{+}(x_{0:T},y_{0:T}),p_{-}(x_{0:T},y_{0:T})])dx_{0:T}.
	\end{eqnarray*}
Exist a sequence of $x_{t,min,i}\in G_i$ ($t=1:T-1$) such that the following lower bound holds.
	This can be further lower bounded by,
	{\small
		\begin{eqnarray*}
			& \geq &
			2^{-(v+1)}\sum_{y_{0:T},w_{0:T}}\sum_{\mathbf{b}}\int_{x_{0:T}}\min[p_{+}(x_{0:T},y_{0:T}),p_{-}(x_{0:T},y_{0:T})]dx_{0:T},\\
			& \geq &
			2^{-(v+1)}\sum_{\mathbf{b}}(\sum_{y_{0:T},w_{0:T}}\int_{x_{0:T}}[p_{+}(x_{0:T},y_{0:T})p_{-}(x_{0:T},y_{0:T})]^{1/2}dx_{0:T})^{2},\\
			& \geq &
			2^{-(v+2)}\sum_{\mathbf{b}}p_{0}(\sum_{y_{t},w_t}\int_{x_t}\P(w_{t})p(x_t|x_{t-1,min,i})\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1,min,i},w_{t})\P_{b_{i+}}(y_{t}|x_{t-1,min,i},w_{t})}dx_{t})^{2(T-1)},\nonumber
	\end{eqnarray*}}
	where the second last last line is due to the LeCam's Inequality, for any positive sequence of $a_i$ and $b_i$, we have,
	\beq
	\sum_i \min(a_i,b_i)\geq 1/2(\sum_i\sqrt{a_i b_i})^2.
	\eeq
	And the last line is by assuming $p(x_{0},y_{0},w_{0})\geq p_{0}$ for any $x_{t-1}\in G$.
	%
%	Now we assume $	\int_{ x_{t-1}\in \times G} p(x_{t}|x_{t-1}) dx_{t-1}dx_t\geq\underline{p}> 0$.
Since we know that only for $x_{t-1}\in G_i$, $\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1})\P_{b_{i+}}(y_{t}|x_{t-1})}$ make the value of
	$\sqrt{1/4-r^2}$. Otherwise it shall take the value of either $1/2 $.
	
	
	Now we can further derive that, for $r\geq 0$,
	\begin{eqnarray*}
		&  &
		\sum_{y_{t}\in\{1/2,-1/2,0\},w_{t}\in\{0,1\}}\int_{x_t}\P(w_{t})p(x_t|x_{t-1,min,i})\sqrt{\P_{b_{i-}}(y_{t}|x_{t-1,min,i})\P_{b_{i+}}(y_{t}|x_{t-1,min,i})}dx_{t}\\
		& \geq & \min\{1/2\bigg(\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\{1/2+1/2\}+2\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\sqrt{1/4-r^{2}}\bigg),\\
				&&1/2\bigg(\int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}+ \int_{x_{t}}p(x_t|x_{t-1,min,i})dx_{t}\bigg)\}\\
& \geq & (1/2+1/2\sqrt{1-4r^{2}}).
%		& \geq & (1/2\underline{p}_1+1/2\underline{p}_2\sqrt{1-4r^{2}}+1/2\underline{p}_1  +1/2 \underline{p}_2),
	\end{eqnarray*}
%	where we assume that $\int_{x_{t}}\int_{x_{t-1}\not\in
%			G_{i}}p(x_t|x_{t-1})dx_{t-1:t}\geq \underline{p}_1>0$ and $\int_{x_{t}}\int_{x_{t-1}\in G_i}p(x_t|x_{t-1})dx_{t-1:t} \geq  \underline{p}_2>0$, and $\underline{p} = \underline{p}_1 + \underline{p}_2$. It is not hard to see that $\underline{p} \geq 1$.
	
	Thus in view of $\sqrt{1-4r^{2}}\geq-4r^{2}+1$, we have
	\begin{eqnarray*}
		E_{i}\geq p_{0}(1-2r^{2})^{2(T-1)}.
	\end{eqnarray*}

So we have
\begin{eqnarray*}
W_T(G^{*}(\mathbf{b}))-W_T(\hat{G})\geq (r/v) p_{0}(1-2r^{2})^{2(T-1)}.
\end{eqnarray*}
Optimize the right hand side with respect to $r$, we take log first, $ \log(r)+\log(p_{0}/v)+2(T-1)\log(1-2r^{2})$.
Take first derivative, we have $r^{-1}+ 2(T-1)(1-2r^2)^{-1} (-4r)=0$. Then we have $r$ is of the order $\sqrt{T-1}^{-1}$.

	
	We take $r=\sqrt{v/(2(T-1))}$, then we have $E_{i}\geq p_{0}(1-v/(T-1))^{2(T-1)}\geq
	p_{0}\{\exp\{-(v/(T-1))/(1-\frac{v}{T-1})\}\}^{2(T-1)}$. So we have $r\sum_{i=1}^{v}E_{i}\geq\sqrt{v/(2(T-1))}\exp(-1)$.
\end{proof}



==> App_proof_Sec6_margin.tex <==
\subsubsection{Proof of Theorem \ref{lem: marginal_improve}} \label{sec: proof_marginal}

%\bea 
%&&\bar{\mathcal{W}}(g,W_{t-2}) \\
%&\defeq&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\E\left\{ Y_{t}(W_{t-1},1)g(W_{t-%1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]|W_{t-2}\right\}. \notag %\label{eq:W2appendix}
%\eea

%\bea 
%&&{\widehat{\mathcal{W}}}(g) \\
%&\defeq&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}%(W_{t-1},0)\left[1-g(W_{t-1})\right]\right\}. \notag \label{eq:W2appendix}
%\eea

%\bea 
%&&{\bar{\mathcal{W}}}(g) \\
%&\defeq&(T-1)^{-1}\sum_{1 \leq t \leq T-1}\E \left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]\right\}. \notag 
%\label{eq:W2appendix}
%\eea

\begin{proof}
Recall the definitions, 
\bea 
\bar{\mathcal{W}}(g|w) 
=T(w)^{-1}\sum_{1 \leq t \leq T-1 : W_{t-1} = w}\E\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]|W_{t-1}\right\}. \notag %\label{eq:W2appendix}
\eea
and 
\bea 
g^*(w) = \argmax_{g(w) \to {0,1}}\bar{\mathcal{W}}(g|w). 
\eea

It is simple to show that, 
$$g^*(.) =  \argmax_{g(w) \to {0,1}}\bar{\mathcal{W}}(g,W_{t-2}). $$
By a similar derivation to  (\ref{welfare_inequality}) and assumption \ref{C.5}, there exists  positive constants $c_w,c'$ such that
\begin{eqnarray*}
&&\bar{\mathcal{W}}(g^*|w)  - \bar{\mathcal{W}}(g|w) \leq 
c_w(\bar{\mathcal{W}}(g^*,W_{t-2})  - \bar{\mathcal{W}}(g,W_{t-2})), \\
&&(\bar{\mathcal{W}}(g^*,W_{t-2})  - \bar{\mathcal{W}}(g,W_{t-2})) \leq c'(\bar{\mathcal{W}}(g^*)  - \bar{\mathcal{W}}(g))  .
\end{eqnarray*}
Therefore, it suffices to look at $\hat{g} = \argmax_{g(w) \to {0,1}} {\widehat{\mathcal{W}}}(g) $.
	Throughout this section we take $\E{_{t-1}}(\cdot) = \E(\cdot| {\mathcal{F}}_{t-2})$, and $\P_{{t-1}}(\cdot)=\text{Pr}(\cdot| {\mathcal{F}}_{t-2})$. $\hat{g}$ is defined as in Section \ref{one-p}.
	
	%	Recall $\bar{ \mathcal{W}}(G) = \frac{1}{T-1}\sum_t\E{_{t-1}} [Y_{t}(1)\IF(X_{t-1} \in G) + Y_{t}(0)\IF(X_{t-1} \not \in G)] $ and
	%	$\widehat{ \mathcal{W}}(G) =  \frac{1}{T-1}\sum_t[Y_{t}(1)\IF(X_{t-1} \in G) \IF(W_t = 1)/ \P(W_t = 1|\mathcal{F}_{t-1}) + Y_{t}(0)\IF(X_{t-1} \not \in G) \IF(W_t = 0)/ \P(W_t = 0|\mathcal{F}_{t-1})] $. We let $\hat{G} = \mbox{argmax}_G \widehat{ \mathcal{W}}(G)$. Therefore $\bar{ \mathcal{W}}(G) - \widehat{ \mathcal{W}}(G)$ are a sum of MDS with respect to the filtration of $\mathcal{F}_{t-1}$.
	
	The first best rule is $\{x: \tau(x)\geq 0\}$.
	Recall that  there exists a positive constant $\overline{P} $ such that $ \frac{1}{T-1}\sum_t \P_{{t-1}} (g^*(W_{t-1})\neq g(W_{t-1}))\geq \overline{P} $ happens with probability $1$, where $\P_{{t-1}}$ is the probability conditional on $\mathcal{F}_{t-2}$.
	We define the set of events $\{A:\min_t |\tau(W_{t-1})|>u \}$.  Then,
	\begin{eqnarray*}
		\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}(g,W_{t-2}) &=& \sum_{1\leq t\leq T-1} \frac{1}{T-1}\E{_{t-1}}\{ |\tau(W_{t-1})||\IF(g^*(W_{t-1})\neq g(W_{t-1}))|\}\\
		&\geq&u\frac{1}{T-1}\sum_{1\leq t\leq T-1} \P_{{t-1}} (g^*(W_{t-1})\neq g(W_{t-1}) \cap  A)\\
		&\geq & u\{\sum_{1\leq t\leq T-1} \frac{1}{T-1}[ \P_{{t-1}} (g^*(W_{t-1})\neq g(W_{t-1}) ) - (u/\eta)^{\alpha}]\},
	\end{eqnarray*}
 where the last inequality is due to Assumption \ref{C.4}.


	
	Set $u= \eta (1+\alpha)^{-1/\alpha} \overline{P}^{1/\alpha} \leq \eta$, then we have
	\begin{eqnarray}
		\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}(g,W_{t-2}) \geq \overline{P}^{(1+\alpha)/\alpha} (1+\alpha)^{-(1+\alpha)/\alpha}\alpha \eta.
	\end{eqnarray}
	
	Let $\Var_{t-1}(.) = \E_{t-1}(.^2) - (\E_{t-1}(.))^2$. From this definition,
	\begin{eqnarray}
		&&\frac{1}{T-1}\sum_{t}\Var{_{t-1}}\{(Y_t(1)- Y_t(0))\IF(g^*(W_{t-1})\neq g(W_{t-1})\} ,\nonumber\\
		&\leq&\frac{1}{T-1}2\sum_{t}\E{_{t-1}}\{(Y_{t}^2(1) + Y_{t}^2(0))\IF(g^*(W_{t-1})\neq g(W_{t-1})\}\nonumber\\
		&& -\frac{1}{T-1}\sum_{t}[\E{_{t-1}}\{(Y_{t}(1)- Y_{t}(0))\IF(g^*(W_{t-1})\neq g(W_{t-1})\}]^2  \nonumber\\
		&\leq& \frac{1}{T-1}\sum_{t}2\E{_{t-1}}\{(Y_{t}^2(1) + Y_{t}^2(0))\IF(g^*(W_{t-1})\neq g(W_{t-1})\}\nonumber\\
		&\leq& (4C^2) (\overline{P})\nonumber\\
		&\leq&(4C^2) (1/ \eta \alpha)^{\alpha/(1+\alpha)} (1+\alpha) (\bar{ \mathcal{W}}(g^*,W_{t-2}) - \bar{ \mathcal{W}}(g,W_{t-2}))^{\alpha/(1+\alpha)},\label{margin}
	\end{eqnarray}
	where the second to last line follows from the bounds imposed on $Y_t(0), Y_{t}(1)$ in Assumption \ref{C.3}, and Assumption \ref{C.5}. The last line is due to Assumption \ref{C.4}.
	
	Next from the Freedman inequality we have, with probability $1-\delta$, for a positive constant $C>2$,
	{\small
		\begin{eqnarray*}
			&&\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}(\hat{g},W_{t-2})\\
			&\leq& (\widehat{ \mathcal{W}}(g^*)- \widehat{ \mathcal{W}}(\hat{g}))
			+\max_{g}|\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}({g},W_{t-2})-( \widehat{ \mathcal{W}}(g^*)-\widehat{ \mathcal{W}}({g}) )|\\
			&\leq&\frac{2\max_{g}\sqrt{\frac{1}{T-1}\sum_t C\Var_{t-1}\{(Y_t(1)- Y_t(0))\IF(g^*(W_{t-1})\neq g(W_{t-1})\}}}{\sqrt{T-1}} \sqrt{\log (2M/\delta)}
			\\&&+ \log (2M/\delta) 2C/(T-1), \\
			&\leq & 2\sqrt{(4C^3)) (1/ \eta \alpha)^{\alpha/(1+\alpha)} (1+\alpha) \max_{g}(\bar{ \mathcal{W}}(g^*,W_{t-2}) - \bar{\mathcal{ W}}({g}, W_{t-2}))^{\alpha/(1+\alpha)}}\sqrt{\log (2M/\delta)}/\sqrt{T-1}
			\\&&+  \log (2M/\delta) 4C/(T-1).
	\end{eqnarray*}}
	The second inequality is due to $\widehat{ \mathcal{W}}(g^*)- \widehat{ \mathcal{W}}(\hat{g}) \leq 0 $, which follows from the definition of $\hat{g}$. The third line is based on (\ref{margin}). Solving the inequality on both sides with respect to $\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}(\hat{g},W_{t-2})$, we have that, with probability $1-\delta$, there exists a positive constant $c_w'$, such that
	\begin{eqnarray*}
	\bar{ \mathcal{W}}(g^*)- \bar{ \mathcal{W}}(\hat{g}) \leq c_w'(\bar{ \mathcal{W}}(g^*,W_{t-2})- \bar{ \mathcal{W}}(\hat{g},W_{t-2})) \lesssim_p  C_{\alpha,\eta,V} (\frac{\sqrt{\log (2/\delta)})}{\sqrt{T-1}})^{2(\alpha+1)/(\alpha+2)},
	\end{eqnarray*}
	Under the stationarity of $X_{t}=\{Y_t,W_t\}$, $C_{\alpha,\eta, V}$ is a constant depending only on $\alpha$, $\eta$, $C$, and $V$.
\end{proof}

==> App_proof_unbounded_M.tex <==
\section{Upper bound for the unbounded welfare function} \label{unbounded}
%\subsection{Unbounded case welfare function}
{\red still based on MDS, need to changed to unconditional bound conditional case. Or probably we could move Theorem  \ref{thm:mds_mean_bound} to the end.}
\begin{assumption}\label{cover2}
	We shall assume that there is a measurable cover which $h(Z.,G) \leq F(Z.)$ for all $G$, and $\max_t |F(Z_t)|_{2,Q}\leq \delta$.
\end{assumption}
\begin{assumption}\label{cover3}
	$\mbox{lim}_{n\to 0}\E{_n}\E\{|F(Z_.)|^2\IF\{|F.| > \sqrt{n}\delta\}\}\to_p 0$.
\end{assumption}
We define the metric $\rho_2(f,g) = (\int|f-g|^2dQ)^{1/2}$.
\begin{assumption}\label{cover4}
	We shall assume that $P (\sigma_n(f,g)/ \rho_2(f,g) >L) \to 0$ as $n \to \infty$, where $\sigma_n(f,g) = n^{-1} (\sum_t \E_{t-1} (f_t-g_t)^2)^{1/2}$.
\end{assumption}
\begin{lemma}\label{unbound}
	Under Assumptions \ref{bound_c}, \ref{unconf_c}, \ref{cover1} to \ref{cover4}, we have
	$$\E|\E{_{n}} h_.|_{\mathcal{H}} \lesssim \delta \sqrt{v/n}.$$
\end{lemma}

\begin{proof}
	We define the truncated functional class $\tilde{\mathcal{H}}^c = \{h\in \mathcal{H}: h^c - \E(h.^c|\mathcal{F}_{.-1})\}$.
	We find that since for $\tilde{h}^c \in  \mathcal{H}^c $  and $\tilde{g}^c \in  \mathcal{H}^c $, we have $\rho_{2,n}(\tilde{h}^c,\tilde{g}^c)\leq \sqrt{2} \sqrt{L+1} \rho_{2,n}(h,g)$ with probability approaching to $1$. Thus $\mathcal{N}(\vps\sqrt{2}\sqrt{L+1}, \mathcal{H}, \rho_{2,n}(.,.)) \lesssim \mathcal{N}(\vps, \mathcal{H}, \rho_{2,n}(.,.))$.
	
	
	We denote $h^c = h(Z_{.},G)\IF\{|h|\leq c\}$. We will apply a truncation argument for $E|nE{_{n}} h_.|_{\mathcal{H}} $, which satisfies
	\begin{eqnarray}
		&&\E{_{n}} h (Z., G)\\ &=& E{_{n}} h(Z.,G) \IF (|h| > c)  +\E{_{n}} h(Z.,G) \IF (|h| \leq c)\nonumber
		\\&&-  \E{_{n}} E{_t} h(Z.,G) \IF (|h| > c) - \E{_{n}} \E{_t} h(Z.,G) \IF (|h| \leq c)
	\end{eqnarray}
	As we have the following bound,
	\begin{eqnarray}
		&&\E{_{n}} |\E{_t }h(Z.,G) \IF (|h| > c) |+ \E{_{n}} |h(Z.,G) \IF (|h| > c)|)\nonumber\\ \leq
		&&\E{_{n}} \E{_t} |F(Z.,G)| \IF (|F| > c)+   \E{_{n}} |F(Z.,G)| \IF (|F| > c).
	\end{eqnarray}
	
	Define the stoping time as $\tau_n = n \vee \max \sigma_k(f,g) \leq L\rho_2(h,g) $.
	
	Then we have the following, with probability approaching 1,
	\begin{eqnarray}
		\sigma_{k}(f^c, g^c) \leq \sigma_{k}(f,g) \leq L \rho_2(h,g).
	\end{eqnarray}
	It hold when $k = \tau_n$ as well.
	For $h^c_. \in \mathcal{H}^c$.
	Thus we have
	\begin{eqnarray*}
		&&\E|n\E{_{n}} h_.|_{\mathcal{H}}  \leq  \E|n(\E{_{n}} h^c_. - \E{_{n}}\E{_t} h^c_.)|_{\mathcal{H}}  \\&&+ n\E\E{_{n}} \E{_t} |F(Z.,G)| \IF (|F| > c)+   n\E\E{_{n}} |F(Z.,G)| \IF (|F| > c)\\
		&&\leq I +II,
	\end{eqnarray*}
	where
	\begin{eqnarray*}
		I &=&\E|n(\E{_{n}} h^c_. - \E{_{n}}\E{_t} h^c_.)|_{\mathcal{H}}
		\\&\leq& \E\{|n(\E{_{n}} h^c_. - \E{_{n}}\E{_t} h^c_.)|_{\mathcal{H}} \IF\{\tau_n = n\} \}+ 2cn\E[\IF\{\tau_n \neq n\}].
	\end{eqnarray*}
	We shall pick $c = \delta \sqrt{n}$, then we can achieve the following bound,
	
	\begin{equation}\label{bounded}
		\E\{n|(\E{_{n}} h^c_. - \E{_{n}}\E{_t} h^c_.)|_{\mathcal{H}} \IF\{\tau_n = n\} \}\lesssim c\int^1_{0} \log \sqrt{\mathcal{N}(\varepsilon, \mathcal{H}, \rho_{n,2}(.,.))}d \varepsilon
	\end{equation}
	
	and $\E[\IF\{\tau_n \neq n\}]  \to 0$ as $n \to \infty$ from Assumption \ref{cover4}.\\
	
	The proof of (\ref{bounded}) shall follow from Lemma \ref{bound}.
	
	
	Let $h^{(0)} = (0,\cdots, 0)$, and the set $B_k : k = 1,\cdots, \overline{K}$. We let $2^{-\overline{K}}\lesssim (\log n)^{-1}$.
	$B_k$ is a cover with radius $2^{-k}\delta$ with the metric $\rho_{2,n}(h,g)$. We denote $h^* = \argmax_{h\in \mathcal{H}} E_n h(Z.,G)$. Let $h^{(k)} = \min_{h \in B_k}\rho_{2,n}(h, h^*) \leq 2^{-k}\delta$.
	Then $\rho_{2,n}(h^{(k)}, h^*) \leq 2^{-k}\delta$ hold for any $h\in B_k$.
	Moreover we have
	\begin{equation}
		\rho_{2,n}(h^{(k-1)}, h^{(k)})\leq \rho_{2,n}(h^{(k-1)}, h^*) + \rho_{2,n}(h^{(k)}, h^*) \leq 3*2^{-k}\delta.
	\end{equation}
	
	We denote $c_k = 2^{-k}c$, $k= 1,\cdots, \overline{K}$ and $c_0= c$. We denote $h^c_k = h\IF\{|h|\leq c_k\}$, and $h^{[c_k,c_{k-1}]}  = h_t\IF\{c_k\leq |h| \leq c_{k-1}\} - E (h_t\IF\{c_k\leq |h| \leq c_{k-1}\}|\mathcal{F}_{t-1}) $.
	By a standard chaining argument, we express any partial sum of  $h^c \in \mathcal{H}^c$ (where $\mathcal{H}^c$ is the space of the truncated  functions $h$ ) by a telescope sum,
	\begin{eqnarray*}
		\sum^{\tau_n}_{i=1} h^c_i(Z_i, G) & \leq & |\sum^{\tau_n}_{i=1}h^{(0)}_{i}| + |\sum^{\overline{K}}_{k=1} \sum^{\tau_n}_{i=1}h_{i}^{(k)c_{k-1}} - h_{i}^{(k-1)c_{k-1}}|+|\sum^{\tau_n}_{i=1}h_{i}^{(\overline{K})c_{\overline{K}}} - h_{i}^{*c_{\overline{K}}}|\\
		&& +|\sum^{\overline{K}}_{k=1} \sum^{\tau_n}_{i=1}h_{i}^{*[c_k,c_{k-1}]} - h_{i}^{(k)[c_k,c_{k-1}]}|.
	\end{eqnarray*}
	
	Thus we have,
	\begin{eqnarray}
		&&\E|\E{_{n}} h_.|_{\mathcal{H}} \leq 2\sum_k^{\overline{K}}\E \max_{f \in B_k , g\in B_{k-1}, \rho_{2}(f,g) \leq 3*2^{-k}*\delta} |\E{_{n}}f^{c_{k-1}}.-g^{c_{k-1}}.|\nonumber\\&&+ \E \max_{f \in B_{\overline{K}} , g\in B_{\overline{K}-1}, \rho_{2}(f,g) \leq 2^{-\overline{K}}*\delta} |\E{_{n}}f^{c_{\overline{K}}}.-g^{c_{\overline{K}}}.|.
	\end{eqnarray}
	To bound the component in the above inequality, we shall apply  Lemma \ref{max} with $A  = 2c_{k-1}$ and $B = L 3 * 2^{-k} \delta n$.
	This is because  on the event $\{\tau_n = n\}$, and a ball of length $3* 2^{-k} \delta$, we shall have with probability approaching $1$,
	\begin{eqnarray*}
		&&\tau_n^{-1}\sum^{\tau_n}_{t=1}\E{_{t-1}}|h_t^c-h_t^{'c}|^2 \leq (2L)\tau_n^{-1}\sum^{\tau_n}_{t=1}\E{_{t-1}}|h_t-h_t'|^2
		\\&&\leq (2L+2)L(d(h_t,h_t'))^2 \leq (2L+2)L (3*2^{-k}\delta)^2.
	\end{eqnarray*}
	Then, one the event $\tau_n = n $ and $\sigma_n(f,g)/ \rho_{2,n}(f,g) \leq L$,
	\begin{eqnarray*}
		&&\E|n\E{_{n}} h^c_. \IF\{\tau_n = n\}|_{\mathcal{H}}\\&& \lesssim \sum^{\overline{K}}_{k=1} (3* 2^{-k} \delta \sqrt{n} \sqrt{L}) \sqrt{\log (1+ 2\mathcal{N}^2(2^{-k}\delta/(\sqrt{2(L+1)}), \mathcal{H}, \rho_{2,n}(.,.)))}\\&& + 2c_{k-1}\log (1+ 2 * \mathcal{N}^2(2^{-k}\delta/(\sqrt{2(L+1)}),\mathcal{H}, \rho_{2,n}(.,.)))\\&&\lesssim \sqrt{n}\int^1_{0} \delta \sqrt{\log ( 2^{1/2} \mathcal{N}(\varepsilon \delta/(\sqrt{2(L+1)}), \mathcal{H}, \rho_{2,n}(.,.) ))}d\varepsilon,
	\end{eqnarray*}
	where $\lesssim$ depends only on $L$.
	
	By Assumption \ref{cover3},
	\begin{eqnarray*}
		II/n &=& \E\E{_{n}} \E{_t} |F(Z.,G)| \IF (|F| > c)+   \E\E{_{n}} |F(Z.,G)| \IF (|F| > c)
		\\&\leq& 2\E\E{_{n}} |F(Z.,G)| \IF (|F| > c) \to 0.
	\end{eqnarray*}
	
	Then the conclusion follows.
\end{proof}

\begin{lemma}{(Concentration)}
	\label{cont1}
	Under Assumption \ref{bound_c}, \ref{unconf_c},, \ref{cover1} and \ref{norm}, with $M$ as a constant, then we have the following bound.
	$$|\E{_{n}} h_.|_{\mathcal{H}} - \E|\E{_{n}} h_.|_{\mathcal{H}} \lesssim_p c_n  \sqrt{v/n}.$$
\end{lemma}
\begin{proof}
	The proof is similar to Lemma \ref{cont} and therefore omitted.
\end{proof}

{\red
	
	\begin{theorem} \label{thm: unbounded upper bound}
		Under  Assumption \ref{bound_c}, \ref{unconf_c}, and \ref{cover1} to \ref{cover4}, we have
		\begin{equation*}
			\underset{P\in\mathcal{P}(M,\kappa)}{\text{sup}}\E\left[|\bar{W}_{p}(G_{p}^{*})-\bar{W}_{p}(\hat{G}_{p})]|\right]\leq C\frac{\delta}{\kappa}\sqrt{\frac{v}{T}}
		\end{equation*}
		
	\end{theorem}
	
	\begin{proof}With the function $h_t$ defined as in (\ref{H_class}), the result follows from (\ref{ub1}), Lemma \ref{bound} and Lemma \ref{cont}.
	\end{proof}
}


==> back_up_2_simple.tex <==
\section{Model and illustrative example} \label{model_example}

%We begin our analysis with a heuristic model with a simple dynamic structure. Through that simple model, 
In this section, we introduce the basic setting, notation, the conditional welfare criterion we aim to maximize, and conditions on the data generating process that are important for the learnability of an optimal policy. Then, we illustrate the main analytical tools used to bound welfare regret through a heuristic model with a simple dynamic structure. 

%Our method motivates from the celebrated work of \cite{manski2004statistical}. We show the connection between our welfare function maximization approach and a few popular decision making tools for dynamic data, e.g. the MDP(Makov Decision Process), and causal analysis based on structural vector autoregression (VAR).

\subsection{Notation, timing, and welfare}
We suppose that the social planner is at the beginning of time $T$. Let $W_t \in \{0, 1 \}$ denote a treatment or policy (e.g., nominal interest rate) implemented at time $t = 0,1,2,\dots$. To simplify the analysis, we assume that $W_t$ is binary (e.g., a high or low interest rate regime). The planner sets $W_T \in \{0, 1\}$, $T \geq 1$, making use the history of observable information up to period $T$ to inform their decision. This observable information consists of an economic outcome (e.g., GDP, unemployment rate, etc.), $Y_{0:T-1}=(Y_0,Y_1,Y_2, \cdots, Y_{T-1})$, the history of implemented policies, $W_{0:T-1}=(W_0,W_1,W_2, \cdots, W_{T-1})$, and covariates other than the policies and the outcome (e.g., inflation), $Z_{0:T-1}=(Z_0, Z_1,Z_2, \cdots, Z_{T-1})$. $Z_t$ can be a multidimensional vector, but both $Y_t$ and $W_t$ are assumed to be univariate. \footnote{It can be extended to the settings with multidimensional outcomes and treatments, where $W_t\in\{0,1\}^{d}$ and $Y_t\in \mathbb{R}^k$. For example, the treatment can be the implementation of government monetary policy, rating agency's change of grade for some asset etc. In the case of network data, treatment comes from an observed network $d=k^{2}$ ($k$ is the number of nodes within the network), for example in social network such as the Facebook, $w_{t}$ is the observed adjacency matrices.}

Following \cite{bojinov2019time}, we refer to a sequence of policies $w_{0:t} = (w_0, w_1, \dots, w_t) \in \{0,1\}^{t+1}$, $t \geq 0$, as a treatment path. A realized treatment path observed in the data $0 \leq t \leq T-1$ is a stochastic process $W_{0:T-1} = (W_0, W_1, \dots, W_{T-1})$ drawn from the data generating process.

 Without loss of generality, we assume that $Z_t$ is generated after the outcome $Y_t$ is observed. The timing of realizations is therefore $$\underset{\text{time period }t-1}{\underbrace{W_{t-1}\to Y_{t-1}\to Z_{t-1}}}\to\underset{\text{time period }t}{\underbrace{W_{t}\to Y_{t}\to Z_{t}}},$$
 i.e., the transition between periods happens after $Z_{t-1}$ is realised but before $W_t$ is realised.\footnote {We do not allow $Z_{t}$ to be realised between $Y_t$ and $W_{t}$. If some $Z$ is realised after $W_{t}$, before $Y_t$ and is not causally effected by $W_t$, the causal link unaffected by placing $Z$ before $W_{t}$ and labeling it $Z_{t-1}$; if this $Z$ is realised after $W_{t}$, before $Y_t$, and is causally effected by $W_t$, then $Z$ is a bad control and should not be included in the model.}

Let
\begin{equation} \label{covariate}
X_{t}=\{W_{t},Y_{t}, Z_{t}^{\prime}\}^{\prime}
\end{equation}
collect the observable variables for period $t$, and let $X_t$ be drawn from $\mathcal{X}$ for $t\in \mathbb{N}$. We define the filtration
{
$$\mathcal{F}_{t-1}=\sigma (X_{0:t-1}),$$ }
where $\sigma(\cdot)$ denotes the Borel $\sigma$-algebra generated by the variables specified in the argument. The filtration $\mathcal{F}_{t-1}$ corresponds to the planner's information set at the time of making their decision in period $T$. 

Following the framework of \cite{bojinov2019time}, we introduce potential outcome time-series. At each $t = 0, 1, 2, \dots,$ and for every treatment path $w_{0:t} \in \{0 ,1 \}^{t+1}$, let $Y_t(w_{0:t}) \in \mathbb{R}$ be the realized period $t$ outcome if the treatment path from $0$ to period $t$ were $w_{0:t}$. Hence, we have a collection of potential outcome paths indexed by treatment path, 
$$
\{ Y_t(w_{0:t}) : w_{0:t} \in \{0, 1 \}^{t+1}, t=0,1,2,\dots \},
$$
which defines $2^{t+1}$ potential outcomes in each period $t$. This is an extension of the Neyman-Rubin causal model originally developed for cross-sectional causal inference. As maintained in \cite{bojinov2019time}, the potential outcomes for each $t$ are indexed by the current and past treatments $w_{0:t}$ only. This imposes the restriction that any future treatment $w_{t+p}$, $p \geq 1$, does not causally affect the current outcome, i.e., an exclusion restriction for future treatments. 

For a realized treatment path $W_{0:t}$, the observed outcome $Y_t$ and the potential outcomes satisfy
$$
Y_t = \sum_{\{w_{0:t} \}} 1 \{W_{0:t-1} = w_{0:t-1} \} Y_t(w_{0:t-1})  
$$
for all $t \geq  0$. 

The baseline setting of the current paper considers the choice of policy $W_T$ for a single period $T$.\footnote{Section \ref{sec_multi} discusses how to extend the single-period policy choice problem to multi-period settings.} We denote the policy choice based on observations up to period $T-1$ by 
\beq \label{eq:policy_f} 
g: \mathcal{X}^{T} \to \{0,1\}.
\eeq
 The period-$T$ treatment is $W_T = g(X_{0:T-1})$, and we refer to $g(\cdot)$ as a \emph{decision rule}. We also define the region in the space of the covariate vector for which the decision rule chooses $W_T =1$ to be 
 \beq \label{gG}
G = \{ X_{0:T-1} : g(X_{0:T-1}) = 1 \} \subset \mathcal{X}^{T},
\eeq
We refer to $G$ as a \emph{decision set}.

We assume that the planner's preferences for period-$T$ are embodied in a social welfare criterion. In particular, we define one-period \emph{welfare conditional on $\mathcal{F}_{T-1}$} (conditional welfare, for short) to be\footnote{Throughout the paper, we acknowledge that the expectation, $\E$, and the probability, $\Pr$, is corresponding to the outer measure whenever a measurability issue is encountered.} 
\bea \label{obj_general}
\mathcal{W}_T(g|\mathcal{F}_{T-1})
&:=& \E \left[ Y_{T}(W_{0:T-1},1) g(X_{0:T-1})+ Y_{T}(W_{0:T-1},0)(1- g(X_{0:T-1}))|\mathcal{F}_{T-1} \right].
\eea 

With some abuse of notation, conditional welfare can be expressed with the decision set $G$ as its argument:
\bea \label{obj_general}
\mathcal{W}_T(G|\mathcal{F}_{T-1})
&:=& \E \left[ Y_{T}(W_{0:T-1},1) 1\{X_{0:T-1} \in G \}+ Y_{T}(W_{0:T-1},0)1\{X_{0:T-1} \notin G \} | \mathcal{F}_{T-1} \right].
\eea

This welfare criterion is conditional on the planner's information set. This contrasts with the unconditonal welfare criterion common in the cross-sectional treatment choice setting, where any conditioning variables (observable characteristics of a units) are averaged out.\footnote{\cite{manski2004statistical} also considers a conditional welfare criterion in the cross-sectional setting.} In the time series setting, it is natural for the planner's preferences to be conditional on the realized history, rather than averaging over realized and unrealized histories, as would be the case if the unconditional criterion were used.

As we clarify in Section \ref{sec:nonpara_conti}, regret for conditional welfare and regret for unconditional welfare require different conditions for convergence, and their rates of convergence may differ. Hence, the existing results for regret convergence for unconditional welfare shown in \cite{kitagawa2018should} do not immediately carry over to the time-series setting.

The planner's optimal policy $g^{\ast}$ maximizes her one-period welfare,
$$
g^{\ast} \in \arg \max_g \mathcal{W}_T(g| \mathcal{F}_{T-1}).
$$
The planner does not know $g^{\ast}$, so she instead seeks a statistical treatment choice rule (\cite{manski2004statistical}) $\hat{g}$, which is a decision rule selected on the basis of the available data $X_{0:T-1}$.

Our goal is to develop a way of obtaining $\hat{g}$ that performs well in terms of the conditional welfare criterion (\ref{obj_general}). Specifically, we assess the statistical performance of an estimated policy rule $\hat{g}$ in terms of the convergence of conditional welfare regret,
\bea \label{cond_regret_general}
\mathcal{W}_T(g^{\ast}|X_{0:T-1} = x_{0:T-1}) - \mathcal{W}_T(\hat{g}|X_{0:T-1} = x_{0:T-1}) 
\eea
and its convergence rate with respect to the sample size $T$. When evaluating realised regret, $X_{0:T-1}$ is set to its realized value in the data. On the other hand, when examining convergence, we accommodate statistical uncertainty over $\hat{g}$ by focusing on convergence with probability approaching one uniformly over a class of sampling distributions for $X_{0:T-1}$. A more precise characterization of the regret convergence results will be given below and in Section \ref{continuous}.  

\subsection{Illustrative model with a discrete covariate} \label{one-p}

We begin our analysis with a simple illustrative  model, which provides a heuristic exposition of the main idea of T-EWM and its statistical properties. We cover more general settings and extensions in Sections \ref{continuous} and \ref{ext}. 

Suppose that the data consists of a bivariate time-series $X_{0:T-1} = ((Y_t,W_t) \in \mathbb{R} \times \{0, 1 \} : t=0,1, \dots, T-1)$ with no other covariates. We impose the following restrictions on the dynamic causal structure and dependence of the observations.

\begin{assumption} \label{ass:toy_example} [Markov properties] The time-series of potential outcomes and observable variables satisfy the following conditions:

(i) \emph{Markovian exclusion}: for $t=2, \dots, T$ and for arbitrary treatment paths $(w_{0:t-2},w_{t-1},w_{t})$ and $(w_{0:t-2}^{\prime},w_{t-1},w_{t})$, where $ w_{0:t-2} \neq w_{0:t-2}^{\prime}$, 
\bea \label{exclu}
Y_t(w_{0:t-2}, w_{t-1},w_{t} ) = Y_t(w_{0:t-2}^{\prime}, w_{t-1},w_{t}) := Y_t(w_{t-1},w_t)
\eea
holds with probability one.

(ii) \emph{Markovian exogeneity}: for $t=1, \dots, T$ and any treatment path $w_{0:t}$,
\bea
Y_t(w_{0:t}) \perp X_{0:t-1} | W_{t-1}.
\eea

(iii) \emph{Markovian assignment}: for $t=1, \dots, T-1$,
\bea
W_t \perp X_{0:t-1} | W_{t-1}.
\eea
\end{assumption}

These assumptions significantly simplify the dynamic structure of the problem. Markovian exclusion, Assumption \ref{ass:toy_example} (i), says that only the current treatment $w_{t}$ and treatment in the previous period $w_{t-1}$ can have a causal impact on the current outcome. This allows the indices of the potential outcomes to be compressed to the latest two treatments $(w_{t-1},w_t)$, as in (\ref{exclu}). Markovian exogeneity, Assumption \ref{ass:toy_example} (ii), states that once you condition on the policy implemented in the previous period $W_{t-1}$, the distribution of the potential outcomes for the current period does not depend on any other past variables. Markovian assignment, Assumption \ref{ass:toy_example} (iii), imposes a similar Markovian restriction for the assignment of policy in all periods up to $T-1$. It is important to note that these assumptions do not impose stationarity: we allow the distribution of potential outcomes to vary across time periods. 

Under Assumption \ref{ass:toy_example},  $\E (Y_{t}(W_{0:t-1})|\mathcal{F}_{t-1})=\E (Y_{t}(W_{t-1},W_t)|W_{t-1}) = \E (Y_{t}|W_{t-1})$. Furthermore, with no loss of conditional welfare, we can reduce the class of policy rules to those that map from $W_{T-1} \in \{0,1 \} $ to $W_T \in \{0,1 \}$, $$g : \{0 , 1\} \to \{0, 1\}.$$
Welfare conditional on $\mathcal{F}_{T-1}$ can then be simplified to
\bea \label{obj_simple}
\mathcal{W}_T(g|W_{T-1})
= \E \{ Y_{T}(W_{T-1},1) g(W_{T-1})+ Y_{T}(W_{T-1},0)(1- g(W_{T-1}))|W_{T-1}\}.
\eea

To make sense of Assumption \ref{ass:toy_example}, we provide a toy example involving vaccination:



\noindent {\bf Example 1.}
Suppose the SP is interested in how the distribution of vaccines affects the chance of  infection/hospitalization/death due to covid-19.
Let $W_t$ denote whether an individual receives a dose of vaccine at period $t$, and $Y_t$ denote the probability of infection/hospitalization/death for this person in period $t$. 
%{\red We want to model $Y_t$'s dependence on $W_t$ (and its lagged terms)}, and we can also model the sequential treatment $W_t$ as a discrete auto-regressive type of process.
For i.i.d. noise $\varepsilon_t$, we assume the following structural equations for the dependence of $Y_t$ on $W_t$ (and its lag) and the dependence of $W_t$ on its lag \footnote{The distribution of $W_{t}$ follows \cite{hamilton1989new}. However, the Markov switching model of \cite{hamilton1989new} has unobserved $W_t$, which differs from this example. } 
\begin{align}
Y_{t} & =\beta_{1}W_{t}+\beta_{2}W_{t-1}+\varepsilon_{t},\label{eq:Yt}\\
W_{t} & =(1-q)+\lambda W_{t-1}+V_{t},\label{eq:Wt}\\
\lambda & =p+q-1, \nonumber \\
 \varepsilon_t & \perp W_{s} \qquad \forall s,t. \label{eq:et} 
 \end{align}
 \begin{align}
\text{If }W_{t-1} & =1,\text{ }\begin{cases}
V_{t}=1-p & \text{with probability }p\\
V_{t}=-p & \text{with probability }1-p,
\end{cases} \label{eq:Vt_1} \\
\text{if }W_{t-1} & =0,\text{ }\begin{cases}
V_{t}=-(1-q) & \text{with probability }q\\
V_{t}=q & \text{with probability }1-q \label{eq:Vt_2}.
\end{cases}
\end{align}

Compatibility with Assumption \ref{ass:toy_example} can be seen as follows. Assumption \ref{ass:toy_example}(i) is implied by \eqref{eq:Yt}; Assumption \ref{ass:toy_example}(ii) is implied by \eqref{eq:Yt}, \eqref{eq:et}, and the fact that the distribution of $V_{t}$ depends solely on $W_{t-1}$; under \eqref{eq:Wt},\eqref{eq:Vt_1}, and \eqref{eq:Vt_2}, we have $\Pr[W_t=1|W_{t-1}=1]=p$, $\Pr[W_t=0|W_{t-1}=1]=1-p$, $\Pr[W_t=0|W_{t-1}=0]=q$, and $\Pr[W_t=1|W_{t-1}=0]=1-q$, so Assumption \ref{ass:toy_example}(iii) is satisfied.\\

%{\bf \color{blue} Remark.}
%We emphasize that the simple illustrative example ({\color{blue} model}) can maintain model-free in the sense that we do not need to specify the function form of $Y_t$ on $W_t$ and $W_{t-1}$. Example 1 is only aimed at helping readers to better understanding assumptions discussed in this section, instead of imposing a parametric structure on our T-EWM framework.\\

To examine the learnability of the optimal policy rule, we further restrict the data generating process. First, we impose a strict overlap condition on the propensity score:
\begin{assumption} \label{bound1} [Strict overlap] Let $e_t(w) := \Pr(W_t = 1|W_{t-1} = w)$ be the period-$t$ propensity score. There exists a constant $\kappa \in (0,1/2)$, such that for any $t = 1, 2, \dots, T-1$ and $w\in \{0,1\}$,
        \begin{equation*}
                \kappa \leq e_t(w) \leq 1-\kappa.
        \end{equation*}
\end{assumption}
The next assumption imposes an unconfoundedness condition on observed policy assignment:
\begin{assumption} \label{unconf} [Unconfoundedness]
        For any $t = 1,2,\dots, T-1$ and $w\in \{0,1\}$,
        \[
        Y_{t}(W_{t-1},w)\perp W_t|X_{0:t-1}.
        \]
\end{assumption}
\noindent {\bf Example 1 continued.} Assumption \ref{bound1} is satisfied if $0<p<1$ and $0<q<1$; Assumption \ref{unconf} is implied by \eqref{eq:Yt} and \eqref{eq:et}.\\

Imposing Assumption \ref{bound1} and \ref{unconf} and assuming propensity scores are known, a sample analogue of (\ref{obj_simple}) conditional on $W_{T-1}=w$ can be constructed
\bea \label{sample_simple}
\widehat{\mathcal{W}}(g|W_{T-1}=w) 
=T(w)^{-1}\sum_{1 \leq t \leq T-1: W_{t-1} = w}[\frac{Y_{t}W_{t}g(W_{t-1})}{e_t(W_{t-1})}+ \frac{Y_{t}(1-W_{t})\{1- g(W_{t-1})\}}{1- e_t(W_{t-1})} ],
\eea
where $T(w) = \#\{1\leq t \leq T-1: W_{t-1} = w\} $ is the number of observations where the policy in the previous period took value $w$, i.e. the subsample corresponding to $W_{t-1} = w$. $\widehat{\mathcal{W}}(g|W_{T-1}=w)$ is the sum of inverse propensity score weighted outcomes over the subsample where the policy of the previous period is restricted to be $W_{T-1}$. We refer to $\widehat{\mathcal{W}}(g|W_{T-1}=w)$ as the empirical welfare of the policy rule $g$.

Denoting $(\cdot|W_{T-1}=w)$ by $(\cdot|w)$, define the true optimal policy and its empirical analogue to be,
\bea 
g^*(w) &\in& \mbox{argmax}_{g: \{w\}\to  \{0,1\}} \mathcal{W}_T(g|w),\label{best_g} \\
\hat{g}(w) &\in& \mbox{argmax}_{g: \{w\}\to  \{0,1\}} \widehat{\mathcal{W}}(g|w).\label{best_g_hat}
\eea
$\hat{g}$ is constructed by maximizing empirical welfare over a class of policy rules (four policy rules in total). We call a policy rule constructed in this way the \textit{Time-series empirical welfare maximization} (T-EWM) rule. The construction of the T-EWM rule $\hat{g}$ is analogous to the conditional empirical success rule with known propensity scores considered by \cite{manski2004statistical} in the i.i.d. cross-sectional setting. In the time-series setting, however, the assumptions imposed so far do not guarantee $\widehat{\mathcal{W}}(g|w)$ is an unbiased estimator of the true conditional welfare $\mathcal{W}_{T}(g|w)$.

\subsection{Bounding the conditional welfare regret of the T-EWM rule} \label{discrete_bound}

A major contribution of this paper is to characterizing conditions that justify the T-EWM rule $\hat{g}$ in terms of the convergence of conditional welfare. This section clarifies these points in the context of our illustrative example. 
%find a upper bound of the population regret. In particular, it is denoted as the difference between the welfare function evaluated at the true policy function and the estimated policy function i.e. \\ $\mathcal{W}_T(g^*|w)- \mathcal{W}_T(\hat{g}|w)$.
 
To bound conditional welfare regret, our strategy is to decompose empirical welfare $\widehat{\mathcal{W}}(g|w)$ into a conditional mean component and a deviation from it. The deviation is the sum of a martingale difference sequence (MDS), and this allows us to apply concentration inequalities for the sum of MDS.  Define an intermediate welfare function,
\bea \label{E_sum_c}
&&\bar{\mathcal{W}}(g|w) \\
&=&T(w)^{-1}\sum_{1 \leq t \leq T-1 : W_{t-1} = w}\E\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]|W_{t-1}\right\}. \notag %\label{eq:W2}
\eea
Under the strict overlap and unconfoundedness assumptions (Assumptions \ref{bound1} and \ref{unconf}), the difference between empirical welfare and  \eqref{E_sum_c} is a MDS. Furthermore, we impose the assumption:
 \begin{assumption}  \label{equiv_W}
        [Invariance of the welfare ordering]\\Given $w\in {0,1}$, let $g^*=g^*(w)$ defined in \eqref{best_g}.   There exist a positive constant $c>0$, such that for any  $g\in\{0,1\}$,
                \bea \label{eq:invariance_toy}
        \mathcal{W}_T(g^*|w)- \mathcal{W}_T(g|w) \leq c\big[\bar{\mathcal{W}}(g^*|w)-\bar{\mathcal{W}}(g|w)\big],
        \eea
        with probability approaching one, i.e., noting that $\bar{\mathcal{W}}(g|w)$ is random as it depends on $W_{0:T-1}$, $P_T \left( \text{inequality (\ref{eq:invariance_toy}) holds} \right) \to 1$ as $T \to \infty$, where $P_T$ is the probability distribution for $X_{0:T-1}$.
\end{assumption}

This assumption guarantees that $\hat{g}$ is consistent for the optimal policy $g^{\ast}$. It states that the welfare ordering of policies for the current period $T$ coincides with the welfare ordering of policies in terms of historical population averages.
\begin{remark} \label{rem:invar_order}
Assumption \ref{equiv_W} can be restrictive in a situation where the dynamic causal structure of the current period is believed to be different from the past, but is weaker than stationarity. In the current example, if we were willing to assume,
        \textit{\begin{description}
                        \item [{A\ref{equiv_W}' }] The stochastic process
                        $$\text{\ensuremath{S_{t}(w)}=\text{\ensuremath{ \ensuremath{Y_{t}}(\ensuremath{W_{t-1}},1)\ensuremath{g}(\ensuremath{W_{t-1}})+\ensuremath{Y_{t}}(\ensuremath{W_{t-1}},0)\ensuremath{\left[1-g(W_{t-1})\right]}|_{\ensuremath{W_{t-1}=w}} } }}$$
                        is weakly stationary.
        \end{description}}
        then, under A\ref{equiv_W}', we would have
        \beaa
        &&\E \{ Y_{T}(W_{T-1},1) g(W_{T-1})+ Y_{T}(W_{T-1},0)(1- g(W_{T-1}))|W_{T-1}=w\} \\
        &=& \E\left\{ Y_{t}(W_{t-1},1)g(W_{t-1})+Y_{t}(W_{t-1},0)\left[1-g(W_{t-1})\right]|W_{t-1}=w\right\} \\
        &=& \E[S_{t}(w)] \text{ for } 2\leq t\leq T.
        \eeaa
        and Assumption (\ref{equiv_W}) would hold naturally.
        \footnote{Assumption \ref{equiv_W} is also weaker than and can be implied by the following assumptions:\\
                The direct one
                \beqq
                \bar{\mathcal{W}}(g|w)=\mathcal{W}_T(g|w).
                \eeqq
                The linear one
                \beqq
                \bar{\mathcal{W}}(g|w)=c_1 \mathcal{W}_T(g|w)+c_2.
                \eeqq
                The asymptotic one
                \beqq
                \bar{\mathcal{W}}(g|w)= \mathcal{W}_T(g|w)+o_p(1/\sqrt{T}).
                \eeqq}
                
  Furthermore,  Assumption \ref{equiv_W} can be satisfied by many classic non-stationary processes in linear time series models, including series with deterministic or stochastic time trends.
  \end{remark}
    \noindent{\bf  Example 1 continued.}\\   
(i) By Remark \ref{rem:invar_order}, Assumption \ref{equiv_W} holds
for Example 1 since
\[
S_{t}(w)=\beta_{1}\cdot g+\beta_{2}\cdot w+\varepsilon_{t}
\]
is weakly stationary. 

$\varepsilon_{t}$ remains an i.i.d. noise in the following settings.

\noindent(ii) If we replace \eqref{eq:Yt} by
\[
Y_{t}=\delta_{t}+\beta_{1}W_{t}+\beta_{2}W_{t-1}+\varepsilon_{t},
\]
where $\delta_{t}$ is an arbitrary deterministic time trend, the
process $Y_{t}$ is trend stationary (non-stationary), but Assumption
\ref{equiv_W} still holds with $c=1$ since those
deterministic trends are canceled out by differences, i.e.,
\[
\mathcal{W}_{T}(g^{*}|w)-\mathcal{W}_{T}(g|w)=\beta_{1}\left(g^{*}-g\right)=\bar{\mathcal{W}}(g^{*}|w)-\bar{\mathcal{W}}(g|w).
\]

\noindent(iii) If we replace \eqref{eq:Yt} by
\[
Y_{t}=\beta_{1}W_{t}+\beta_{2}W_{t-1}+\sum_{i=0}^{t}\varepsilon_{i},
\]
the process $Y_{t}$ is non-stationary with stochastic trends, but
Assumption \ref{equiv_W} still holds with $c=1$
since the stochastic trends are canceled out by differences.

\noindent(iv) If we replace \eqref{eq:Yt} by
\[
Y_{t}=\beta_{1,t}W_{t}+\beta_{2,t}W_{t-1}+\varepsilon_{t}
\]
to allow heterogeneous treatment effect. Then
\begin{align*}
\mathcal{W}_{T}(g^{*}|w)-\mathcal{W}_{T}(g|w) & =\beta_{1,T}\left(g^{*}-g\right)\\
\bar{\mathcal{W}}(g^{*}|w)-\bar{\mathcal{W}}(g|w) & =\bar{\beta}_{w}\left(g^{*}-g\right),
\end{align*}
where $\bar{\beta}_{w}:=\frac{1}{T(w)}\sum_{1\leq t\leq T-1:W_{t-1}=w}\beta_{1,t}$.
Since $\mathcal{W}_{T}(g^{*}|w)-\mathcal{W}_{T}(g|w)$ is non-negative
by the definition of $g^{*}$ in  \eqref{best_g}, Assumption \ref{equiv_W}
holds if 
$$\text{$\beta_{1,T}$ and $\bar{\beta}_{w}$ have the same
sign and $c\geq\frac{|\beta_{1,T}|}{|\bar{\beta}_{w}|}.$}$$
Without loss of generality, we can assume that both $\beta_{1,T}$
and $\bar{\beta}_{w}$ are positive, then a sufficient condition for Assumption \ref{equiv_W} is: There
are positive number $l$ and $u$, such that $0<l\leq\beta_{1,t}\leq u$
holds for all $t$. In this case, $c=\frac{u}{l}$.\\
    
 Assumption \ref{equiv_W} implies that $g^*$ also maximizes $\bar{\mathcal{W}}$. Hence, if empirical welfare $\widehat{\mathcal{W}}(\cdot|w)$ can approximate $\bar{\mathcal{W}}(\cdot|w)$ well, intuitively the T-EWM rule $\hat{g}$ should converge to $g^{\ast}$. 
 
 The motivation for Assumption \ref{equiv_W} is to create a bridge between $\mathcal{W}_{T}(g^*|w)-\mathcal{W}_{T}(\hat{g}|w)$, the population regret,  and $\widehat{\mathcal{W}}(\cdot|w) - \bar{\mathcal{W}}(\cdot|w) $, which is a sum of MDS  with respect to filtration $\{ \mathcal{F}_{t-1} : t = 1,2, \dots, T \}$.\footnote{Note in the current simple example, $\E(\cdot|\mathcal{F}_{t-1})=\E(\cdot|W_{t-1} )$.}
 Specifically, 
  \begin{align} \label{ineq_s}
        & \mathcal{W}_{T}(g^*|w)-\mathcal{W}_{T}(\hat{g}|w)\nonumber\\
        \leq & c\left[\bar{\mathcal{W}}(g^*|w)-\bar{\mathcal{W}}(\hat{g}|w)\right]\nonumber\\
        = & c\left[\bar{\mathcal{W}}(g^*|w)-\widehat{\mathcal{W}}(\hat{g}|w)+\widehat{\mathcal{W}}(\hat{g}|w)-\bar{\mathcal{W}}(\hat{g}|w)\right]\nonumber\\
        \leq & c\left[\bar{\mathcal{W}}(g^*|w)-\widehat{\mathcal{W}}(\tilde{g}|w)+\widehat{\mathcal{W}}(\hat{g}|w)-\bar{\mathcal{W}}(\hat{g}|w)\right]\nonumber\\
        \leq & 2c\sup_{g:\{w\}\to  \{0,1\}}|\bar{\mathcal{W}}(g|w)-\widehat{\mathcal{W}}(g|w)|,
 \end{align}
 where the first inequality follows by Assumption \ref{equiv_W}. The second inequality follows from the definition of T-EWM rule $\hat{g}$ in \eqref{best_g_hat}.

 To bound the right-hand side of \eqref{ineq_s}, define
 \beaa
 \widehat{\mathcal{W}}_t(g|w)=1(W_{t-1}=w)\left[\frac{Y_{t}W_{t}g(W_{t-1})}{e_t(W_{t-1})}+ \frac{Y_{t}(1-W_{t})\{1- g(W_{t-1})\}}{1- e_t(W_{t-1})}\right],
 \eeaa
 and
 \beaa
\bar{\mathcal{W}}_t(g|w)=1(W_{t-1}=w)\E \{ Y_{t}(W_{t-1},1) g(W_{t-1})+ Y_{t}(W_{t-1},0)(1- g(W_{t-1}))|W_{t-1}=w\}.
 \eeaa
 We then express \eqref{sample_simple} and \eqref{E_sum_c} as
 \beaa
 \widehat{\mathcal{W}}(g|w)
 =&\frac{T-1}{T(w)}\cdot \frac{1}{T-1}\sum_{t  = 1}^{T-1}\widehat{\mathcal{W}}_t(g|w),\\
\bar{\mathcal{W}}(g|w)
 =&\frac{T-1}{T(w)}\cdot \frac{1}{T-1}\sum_{t  = 1}^{T-1}\bar{\mathcal{W}}_t(g|w),
 \eeaa
 and
 \bea
 \widehat{\mathcal{W}}(g|w) - \bar{\mathcal{W}}(g|w) = \frac{T-1}{T(w)} \cdot \frac{1}{T-1} \sum_{t=1}^{T-1} \left[ \widehat{\mathcal{W}}_t(g|w) - \bar{\mathcal{W}}_t(g|w) \right] \notag
 \eea
 follows. By Assumption \ref{unconf}, $\widehat{\mathcal{W}}_t(g|w)-\bar{\mathcal{W}}_t(g|w)$ is a MDS, so  we can apply a concentration inequality for sums of MDS to obtain a high-probability bound for $\widehat{\mathcal{W}}(g|w) - \bar{\mathcal{W}}(g|w)$ that is uniform in $g$.  
 
 Specifically, in Appendix \ref{simple_mds_proof} we show that
 \begin{equation} \label{simp_rate}
        \sup_{g: \{0,1\}\to \{0,1\}}\left\{\widehat{\mathcal{W}}(g|w) - \bar{\mathcal{W}}(g|w)\right\} \lesssim_p \frac{C}{\sqrt{T-1}},
 \end{equation}
where $C$ is a constant defined in the proof and $\lesssim_p$ denotes an upper bound valid with (upper) probability approaching one. That is, for a random sequence $A_{T}$ that follows an (outer) probability measure
$P_{T}$ and a deterministic sequence $\varepsilon_T$, $T=1,2,3, \dots$, $A_T \lesssim_{p} \varepsilon_T$ means that there exists a positive constant $c$ such that,
\[
P_T(A_{T}>c\varepsilon_T)\overset{T\to\infty}{\to}0.
\]
  Combining (\ref{ineq_s}) and (\ref{simp_rate}), we can conclude that the convergence rate of regret $\mathcal{W}_{T}(g^*|w)-\mathcal{W}_{T}(\hat{g}|w)$ is of order $O_p(\frac{1}{\sqrt{T-1}})$, and is uniform in the conditioning value of $w$.
  

==> optimality_section.tex <==
\section{Optimal Decision Theory: Convolution Theorem and Local Asymptotic Minimax}
\label{sec:optimality}

This section derives the decision-theoretic optimality of the plug-in
causal estimator $\hat\mu = \hat\lambda_{i_0,1}\,\hat F_{T+1,1}$ for the
counterfactual functional $\mu_0 = \lambda_{i_0,1}^0 F_{T+1,1}^0$. The
analysis proceeds in three steps: (i) the convolution theorem of H\'{a}jek
(1970) and Le Cam (1972), restricting the limit law of any regular
estimator; (ii) the local asymptotic minimax theorem, providing a sharp
lower bound on local risk for any measurable estimator and any
subconvex loss; and (iii) the achievement result, showing that $\hat\mu$
attains the bound. Together these establish that $\hat\mu$ is locally
asymptotically minimax optimal in the semiparametric model with
infinite-dimensional nuisance.

The framework follows van der Vaart (1998, Chapter~25), specialized to
the panel-factor setting via the LAN expansion of
Theorem~\ref{thm:lan}.

\subsection{Regular Estimators and the Convolution Theorem}
\label{subsec:convolution}

\begin{definition}[Regular estimator]
\label{def:regular}
A sequence of estimators $\{\hat\mu_{NT}\}$ of $\mu_0$ is
\emph{regular} at $P_0$ relative to the local sequence
\eqref{eq:local_param} if there exists a (tight) probability law $L$ on
$\mathbb{R}$ such that for every $h \in \mathbb{R}$,
\begin{equation}
  \sqrt{T}\bigl(\hat\mu_{NT} - \mu_{NT}(h)\bigr)
  \;\xrightarrow{d}\; L
  \qquad\text{under } P_{NT,h}.
  \label{eq:regular}
\end{equation}
That is, the limit law $L$ does not depend on the local parameter $h$.
\end{definition}

\begin{remark}[Interpretation of regularity]
\label{rem:regularity}
Regularity is a uniformity requirement: the estimator's centered limit
distribution is invariant under local reparametrization. Most reasonable
estimators in semiparametric models are regular under standard
conditions; pathological exceptions such as Hodges' superefficient
estimator violate regularity and pay for their pointwise improvement
with poor uniform behavior. The convolution theorem constrains regular
estimators only; the local asymptotic minimax theorem of
Section~\ref{subsec:lam} dispenses with regularity by considering
worst-case local risk over shrinking neighborhoods.
\end{remark}

\begin{theorem}[Convolution theorem]
\label{thm:convolution}
Under Assumptions~\ref{ass:model}--\ref{ass:rate} and the LAN expansion
\eqref{eq:lan}, any regular estimator $\hat\mu_{NT}$ of $\mu_0$
satisfies
\begin{equation}
  L \;=\; \mathcal{N}(0,\, V_{\mathrm{eff}}) \,\star\, M
  \label{eq:convolution}
\end{equation}
for some probability measure $M$ on $\mathbb{R}$, where $V_{\mathrm{eff}}$
is the semiparametric information bound \eqref{eq:V_eff} and $\star$
denotes convolution. In particular, the asymptotic variance of any
regular estimator satisfies
\begin{equation}
  \mathrm{Var}(L) \;\geq\; V_{\mathrm{eff}},
  \label{eq:var_bound}
\end{equation}
with equality if and only if $M = \delta_0$, in which case $\hat\mu_{NT}$
is asymptotically efficient.
\end{theorem}

\begin{proof}
By Theorem~\ref{thm:lan}, the experiment $\{P_{NT,h} : h \in \mathbb{R}\}$
converges to the Gaussian shift experiment $\{\mathcal{N}(h, V_{\mathrm{eff}})
: h \in \mathbb{R}\}$ in the sense of Le Cam. Apply the convolution
theorem (van der Vaart, 1998, Theorem~25.20): for any regular sequence
of estimators with limit law $L$ in this experiment,
$L = \mathcal{N}(0, V_{\mathrm{eff}}) \star M$ for some distribution
$M$. The variance bound \eqref{eq:var_bound} follows because
convolution increases variance, with equality if and only if $M$ is a
point mass at zero.
\end{proof}

\subsection{Local Asymptotic Minimax Bound}
\label{subsec:lam}

The convolution theorem applies only to regular estimators. The local
asymptotic minimax (LAM) theorem provides a sharper conclusion that
holds for every measurable estimator, by passing to a sup over local
neighborhoods.

\begin{definition}[Subconvex loss]
\label{def:loss}
A loss function $\ell: \mathbb{R} \to [0,\infty)$ is \emph{subconvex} if
its sublevel sets $\{x : \ell(x) \leq c\}$ are convex and symmetric
about the origin for every $c \geq 0$.
\end{definition}

Examples: $\ell(x) = x^2$ (squared-error), $\ell(x) = |x|$ (absolute
error), $\ell(x) = \mathbf{1}\{|x| > c\}$ (indicator of interval). All
common losses in econometric practice are subconvex.

\begin{theorem}[Local asymptotic minimax bound]
\label{thm:lam}
Under Assumptions~\ref{ass:model}--\ref{ass:rate} and the LAN expansion
\eqref{eq:lan}, for any subconvex loss $\ell$ and any sequence of
measurable estimators $\hat\mu_{NT}$ of $\mu_0$,
\begin{equation}
  \liminf_{c\to\infty}\;\liminf_{NT\to\infty}\;
  \sup_{|h|\leq c}\;
  \mathbb{E}_{P_{NT,h}}\!\Bigl[\ell\bigl(\sqrt{T}(\hat\mu_{NT} - \mu_{NT}(h))\bigr)\Bigr]
  \;\geq\; \mathbb{E}\bigl[\ell(Z)\bigr],
  \label{eq:lam_bound}
\end{equation}
where $Z \sim \mathcal{N}(0,\, V_{\mathrm{eff}})$ and $V_{\mathrm{eff}}$
is the semiparametric information bound \eqref{eq:V_eff}.
\end{theorem}

\begin{proof}
The Gaussian shift limit experiment $\{\mathcal{N}(h, V_{\mathrm{eff}})
: h \in \mathbb{R}\}$ has minimax risk $\mathbb{E}[\ell(Z)]$ for
estimating $h$ under any subconvex loss, attained by the identity
estimator $\hat h = X$ (van der Vaart, 1998, Theorem~8.11; this is
Anderson's lemma applied to Gaussian translation families). By the LAN
convergence of Theorem~\ref{thm:lan} and the asymptotic minimax theorem
(van der Vaart, 1998, Theorem~25.21), this minimax risk is the
asymptotic lower bound for the original experiment, yielding
\eqref{eq:lam_bound}.
\end{proof}

\begin{remark}[Squared-error special case]
\label{rem:squared_error}
Specializing to $\ell(x) = x^2$, Theorem~\ref{thm:lam} gives
\begin{equation}
  \liminf_{c\to\infty}\;\liminf_{NT\to\infty}\;
  \sup_{|h|\leq c}\;
  T\,\mathbb{E}_{P_{NT,h}}\!\bigl[(\hat\mu_{NT} - \mu_{NT}(h))^2\bigr]
  \;\geq\; V_{\mathrm{eff}},
  \nonumber
\end{equation}
i.e., the local asymptotic worst-case mean squared error of any
estimator is at least $V_{\mathrm{eff}}/T$. This is the strongest
possible lower bound in the absence of additional structure on the
estimator class.
\end{remark}

\subsection{Achievement: The Plug-in Estimator Attains the Bound}
\label{subsec:achievement}

The plug-in causal estimator is
\begin{equation}
  \hat\mu \;=\; \hat\lambda_{i_0,1}\,\hat F_{T+1,1},
  \label{eq:plugin}
\end{equation}
where $(\hat\lambda_{i_0,1}, \hat F_{T+1,1})$ are the maximum likelihood
estimators of the corresponding scalar coordinates, obtained via
penalized maximum likelihood under the Bai normalization
\eqref{ass:normalization}. The asymptotic distribution of $\hat\mu$
follows from the asymptotic linear representations of
Theorem~\ref{thm:alr}, applied to each scalar component, plus the delta
method for the bilinear functional.

\begin{theorem}[Asymptotic distribution and efficiency of $\hat\mu$]
\label{thm:achievement}
Under Assumptions~\ref{ass:model}--\ref{ass:rate}, the plug-in causal
estimator \eqref{eq:plugin} satisfies
\begin{equation}
  \sqrt{T}\bigl(\hat\mu - \mu_0\bigr)
  \;\xrightarrow{d}\;
  \mathcal{N}\bigl(0,\, V_{\mathrm{eff}}\bigr),
  \label{eq:plugin_normal}
\end{equation}
where $V_{\mathrm{eff}}$ is the semiparametric information bound
\eqref{eq:V_eff}. Moreover, $\hat\mu$ is regular in the sense of
Definition~\ref{def:regular} and is therefore asymptotically efficient
according to the convolution theorem (Theorem~\ref{thm:convolution})
and the LAM theorem (Theorem~\ref{thm:lam}).
\end{theorem}

\begin{proof}
By Theorem~\ref{thm:alr}, the maximum likelihood estimators admit the
asymptotic linear representations
\begin{align}
  \hat\lambda_{i_0,1} - \lambda_{i_0,1}^0
  &\;=\; \frac{1}{\mathcal{J}_{i_0}^F}\sum_{t=1}^{T} s_{i_0 t}\,F_{t1}^0
       + O_p(\delta_{NT}^{-2}),
  \nonumber\\
  \hat F_{T+1,1} - F_{T+1,1}^0
  &\;=\; \frac{1}{\mathcal{J}_{T+1}^\Lambda}\sum_{i=1}^{N} s_{i,T+1}\,\lambda_{i1}^0
       + O_p(\delta_{NT}^{-2}).
  \nonumber
\end{align}
Apply the delta method to the bilinear map $\mu(a,b) = a\cdot b$ at
$(\lambda_{i_0,1}^0, F_{T+1,1}^0)$:
\begin{align}
  \hat\mu - \mu_0
  &\;=\; F_{T+1,1}^0\,(\hat\lambda_{i_0,1} - \lambda_{i_0,1}^0)
       + \lambda_{i_0,1}^0\,(\hat F_{T+1,1} - F_{T+1,1}^0)
       + O_p\bigl(\delta_{NT}^{-2}\bigr) \nonumber\\
  &\;=\; F_{T+1,1}^0\,\frac{\phi_{i_0,1}}{\mathcal{J}_{i_0}^F}
       + \lambda_{i_0,1}^0\,\frac{\psi_{T+1,1}}{\mathcal{J}_{T+1}^\Lambda}
       + O_p\bigl(\delta_{NT}^{-2}\bigr) \nonumber\\
  &\;=\; \tilde\ell_\mu + O_p\bigl(\delta_{NT}^{-2}\bigr),
  \label{eq:alr_mu}
\end{align}
where the second equality uses the definition of the orthogonalized
scores $\phi_{i_0,1}$ and $\psi_{T+1,1}$, and the third equality
identifies the leading term as the efficient influence function from
\eqref{eq:eif}.

Multiplying by $\sqrt{T}$ and applying the central limit theorem
(under Assumptions~\ref{ass:score_moments} and \ref{ass:score_reg};
see proof of Theorem~\ref{thm:lan}):
\[
  \sqrt{T}(\hat\mu - \mu_0)
  \;=\; \sqrt{T}\,\tilde\ell_\mu + o_p(1)
  \;\xrightarrow{d}\; \mathcal{N}(0, V_{\mathrm{eff}}),
\]
where the variance is computed via Corollary~\ref{cor:info_bound}.

For regularity, observe that under the local sequence $\theta_{NT}(h)$,
the same expansion holds with $\mu_0$ replaced by $\mu_{NT}(h) = \mu_0
+ h/\sqrt{T}$ and the score $s_{it}$ replaced by its evaluation at the
local index. Le Cam's third lemma (van der Vaart, 1998, Example~6.7)
implies that under $P_{NT,h}$,
\[
  \sqrt{T}(\hat\mu - \mu_{NT}(h))
  \;\xrightarrow{d}\; \mathcal{N}(0, V_{\mathrm{eff}})
  \qquad\text{for every } h \in \mathbb{R}.
\]
The limit law does not depend on $h$, establishing regularity.

Asymptotic efficiency follows from Theorem~\ref{thm:convolution}: the
limit variance equals the convolution-theorem lower bound
$V_{\mathrm{eff}}$, so the noise component $M$ in
\eqref{eq:convolution} is a point mass at zero.
\end{proof}

\subsection{Optimality Statement}
\label{subsec:optimality}

Combining the LAM lower bound (Theorem~\ref{thm:lam}) with the
achievement result (Theorem~\ref{thm:achievement}) yields the master
decision-theoretic optimality statement.

\begin{theorem}[Local asymptotic minimax optimality]
\label{thm:optimality}
Under Assumptions~\ref{ass:model}--\ref{ass:rate} and the Bai
normalization \eqref{ass:normalization}, the plug-in causal estimator
$\hat\mu = \hat\lambda_{i_0,1}\,\hat F_{T+1,1}$ is locally
asymptotically minimax optimal for $\mu_0 = \lambda_{i_0,1}^0 F_{T+1,1}^0$
in the semiparametric model with infinite-dimensional nuisance $\eta =
(\lambda_{-i_0,1}, f_1, \Lambda_{-1}, F_{-1})$. Specifically, for any
subconvex loss $\ell$,
\begin{equation}
  \lim_{NT\to\infty}\,\sup_{|h|\leq c}\,
  \mathbb{E}_{P_{NT,h}}\!\Bigl[\ell\bigl(\sqrt{T}(\hat\mu - \mu_{NT}(h))\bigr)\Bigr]
  \;=\; \mathbb{E}\bigl[\ell(Z)\bigr]
  \label{eq:optimality_attainment}
\end{equation}
for every $c > 0$, where $Z \sim \mathcal{N}(0, V_{\mathrm{eff}})$, and
this value coincides with the LAM lower bound from
Theorem~\ref{thm:lam}. Consequently, no measurable estimator
$\hat\mu_{NT}^*$ can achieve strictly smaller asymptotic worst-case
local risk than $\hat\mu$ over $\{|h| \leq c\}$ as $c \to \infty$ and
$NT \to \infty$.
\end{theorem}

\begin{proof}
The upper bound \eqref{eq:optimality_attainment} follows from
Theorem~\ref{thm:achievement}: by regularity, $\sqrt{T}(\hat\mu -
\mu_{NT}(h)) \xrightarrow{d} \mathcal{N}(0, V_{\mathrm{eff}})$ uniformly
on $\{|h| \leq c\}$, and continuous mapping plus dominated convergence
deliver convergence of expectations. The lower bound is
Theorem~\ref{thm:lam}. The two coincide.
\end{proof}

\subsection{Variance Estimation and Confidence Intervals}
\label{subsec:variance}

For inference, $V_{\mathrm{eff}}$ must be estimated. A consistent
plug-in estimator is
\begin{equation}
  \hat V_{\mathrm{eff}}
  \;=\; \hat F_{T+1,1}^2 \cdot
        \Biggl(\sum_{t=1}^{T} \hat{\mathcal{I}}_{i_0 t}\,\hat F_{t1}^2\Biggr)^{-1}
        + \hat\lambda_{i_0,1}^2 \cdot
        \Biggl(\sum_{i=1}^{N} \hat{\mathcal{I}}_{i,T+1}\,\hat\lambda_{i1}^2\Biggr)^{-1},
  \label{eq:V_eff_hat}
\end{equation}
where $\hat{\mathcal{I}}_{it} = -\partial_\pi^2\ell_{it}(\hat\pi_{it})$
is the plug-in observation-level Fisher information. Under
Assumptions~\ref{ass:loglik} and \ref{ass:fisher} and the consistency
of $(\hat\Lambda, \hat F)$ established in Theorem~\ref{thm:alr},
$\hat V_{\mathrm{eff}} \xrightarrow{p} V_{\mathrm{eff}}$.

\begin{corollary}[Asymptotic confidence intervals]
\label{cor:confidence}
Under the assumptions of Theorem~\ref{thm:optimality}, an asymptotic
$(1-\alpha)$-confidence interval for $\mu_0$ is
\begin{equation}
  \mathrm{CI}_{1-\alpha}
  \;=\; \biggl[\,\hat\mu \;\pm\; z_{1-\alpha/2}\sqrt{\hat V_{\mathrm{eff}}/T}\,\biggr],
  \label{eq:CI}
\end{equation}
where $z_{1-\alpha/2}$ is the $(1-\alpha/2)$-quantile of the standard
normal distribution. This interval has the smallest possible asymptotic
length among all regular confidence intervals achieving coverage
$1-\alpha$.
\end{corollary}

\begin{proof}
Coverage follows from \eqref{eq:plugin_normal} and consistency of
$\hat V_{\mathrm{eff}}$ via Slutsky's theorem. The optimality of the
length follows from the fact that any regular interval has asymptotic
length at least $2 z_{1-\alpha/2}\sqrt{V_{\mathrm{eff}}/T}$ by the
convolution theorem applied to the corresponding regular point
estimator (van der Vaart, 1998, Section~25.6).
\end{proof}

\subsection{Discussion}
\label{subsec:discussion}

\paragraph{Comparison with parametric optimality.}
The local asymptotic minimax framework specializes to classical
Cram\'{e}r--Rao optimality when the nuisance parameter is
finite-dimensional and the model is regular (van der Vaart, 1998,
Theorem~8.11). The novel content of Theorem~\ref{thm:optimality} is
that the same conclusion holds when the nuisance is infinite-dimensional,
provided the orthogonalization of Section~\ref{sec:ortho} permits
explicit computation of the efficient influence function. The
asymptotic block diagonality of Wang (2021)
(Theorem~\ref{thm:block_diag}) is the structural fact that makes this
possible in the panel-factor setting.

\paragraph{Comparison with global minimax.}
Theorem~\ref{thm:optimality} is a \emph{local} minimax statement: the
sup is taken over local neighborhoods $\{|h| \leq c\}$ shrinking at
rate $1/\sqrt{T}$ around the true parameter. Global minimax statements
(without the local restriction) typically fail to admit non-trivial
estimators in semiparametric models because the worst-case parameter
can place the nuisance in pathological configurations. The local
restriction is the standard semiparametric remedy and is what makes
optimality results meaningful in practice.

\paragraph{Causal interpretation.}
The decision-theoretic optimality of $\hat\mu$ is a statement about
estimation efficiency for the parameter $\mu_0 = \lambda_{i_0,1}^0
F_{T+1,1}^0$ within the data-generating model. Its interpretation as a
causal effect (e.g., a counterfactual outcome under the synthetic
control framework) requires a separate identification argument
linking $\mu_0$ to a causal estimand of interest. Under the
identification assumptions maintained in this paper,
Theorem~\ref{thm:optimality} certifies that $\hat\mu$ is the best
possible estimator of the identified causal parameter, in the local
asymptotic minimax sense, among all measurable estimators using the
panel data $\{x_{it}\}_{i\leq N, t\leq T}$.

\paragraph{Extensions.}
The same framework extends to vector-valued functionals $\mu(\theta) =
(\lambda_{i_0,1}F_{T+1,1}, \ldots, \lambda_{i_K,1}F_{T+K,1})$ for
multiple targets, with $V_{\mathrm{eff}}$ replaced by the corresponding
efficient information matrix. Treatment-effect functionals of the form
$\mu = g(\lambda_{i_0,1}F_{T+1,1}, \lambda_{j_0,1}F_{T+1,1})$ for smooth
$g$ are handled by the delta method as in Theorem~\ref{thm:achievement}.
Both extensions preserve the local asymptotic minimax optimality of the
plug-in MLE.

